Multiparty Routing: Secure Routing for Mixnets

Anonymous communication networks are important building blocks for online privacy protection. One approach to achieve anonymity is to relay messages through multiple routers, where each router shuffles messages independently. To achieve anonymity, at least one router needs to be honest. In the presence of an adversary that is controlling a subset of the routers unbiased routing is important for guaranteeing anonymity. However, the routing strategy also influenced other factors such as the scalability and the performance of the system. One solution is to use a fixed route for relaying all messages with many routers. If the route is not fixed the routing decision can either be made by the communication initiator or the intermediate routers. However, the existing routing types each have limitations. For example, one faces scalability issues when increasing the throughput of systems with fixed routes. Moreover, when the routing decision is left to the initiator, the initiator needs to maintain an up-to-date view of the system at all times, which also does not scale. If the routing decision is left to intermediate routers the routing of the communication can be influenced by an adversary. In this work, we propose a novel multiparty routing approach for anonymous communication that addresses these shortcomings. We distribute the routing decision and verify the correctness of routing to achieve routing integrity. More concretely, we provide a mixnet design that uses our routing approach and that in addition, addresses load balancing. We show that our system is secure against a global active adversary.

==> references.tex <==

@misc{Tor:2016:website,
  title = {{T}or {P}roject: {A}nonymity {O}nline},
  howpublished = {\url{https://www.torproject.org/}},
  note = {Last accessed: July 30, 2017}
}


@article{Troncoso:2017:Decentralization,
  title={Systematizing Decentralization and Privacy: Lessons from 15 years of research and deployments},
  author={Troncoso, Carmela and Danezis, George and Isaakidis, Marios and Halpin, Harry},
  journal={arXiv preprint arXiv:1704.08065},
  year={2017}
}

@Inbook{Alon:2016:OptimalCointTossing,
author={Alon, Bar and Omri, Eran},
editor={Hirt, Martin and Smith, Adam},
title={Almost-Optimally Fair Multiparty Coin-Tossing with Nearly Three-Quarters Malicious},
bookTitle={Theory of Cryptography: 14th International Conference, TCC 2016-B, Beijing, China, October 31-November 3, 2016, Proceedings, Part I},
year={2016},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={307--335},
isbn={978-3-662-53641-4},
doi={10.1007/978-3-662-53641-4_13},
url={https://doi.org/10.1007/978-3-662-53641-4_13}
}


@misc{Chaum:2016:cMix,
    author = {David Chaum and Debajyoti Das and Farid Javani and Aniket Kate and Anna Krasnova and Joeri de Ruiter and Alan T. Sherman },
    title = {c{M}ix: Anonymization by {H}igh-{P}erformance {S}calable {M}ixing},
    howpublished = {Cryptology ePrint Archive, Report 2016/008},
    year = {2016},
    note = {\url{http://eprint.iacr.org/}},
}


@inproceedings{Kuesters:2016:sElect,
  author = {Ralf K{\"u}sters and Johannes M{\"u}ller and Enrico Scapin and 
Tomasz Truderung},
  title = {{sElect: A Lightweight Verifiable Remote Voting System}},
  booktitle = {{IEEE} 29th Computer Security Foundations Symposium, {CSF} 2016},
  year = 2016,
  publisher = {IEEE Computer Society},
}

@Article{Moran:2016:OptimalCoinToss,
author={Moran, Tal and Naor, Moni and Segev, Gil},
title={An Optimally Fair Coin Toss},
journal={Journal of Cryptology},
year={2016},
volume={29},
number={3},
pages={491--513},
issn={1432-1378},
doi={10.1007/s00145-015-9199-z},
url={http://dx.doi.org/10.1007/s00145-015-9199-z}
}


@article{Kwon:2016:Riffle,
  author    = {Albert Kwon and
               David Lazar and
               Srinivas Devadas and
               Bryan Ford},
  title     = {Riffle: An Efficient Communication System With Strong Anonymity},
  journal   = {PoPETs},
  volume    = {2016},
  number    = {2},
  pages     = {115--134},
  year      = {2016},
  url       = {http://www.degruyter.com/view/j/popets.2015.2016.issue-2/popets-2016-0008/popets-2016-0008.xml},
  timestamp = {Tue, 14 Jun 2016 17:21:11 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/popets/KwonLDF16},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@article{Kwon:2016:Atom,
  title={Atom: Scalable Anonymity Resistant to Traffic Analysis},
  author={Kwon, Albert and Corrigan-Gibbs, Henry and Devadas, Srinivas and Ford, Bryan},
  journal={arXiv preprint arXiv:1612.07841},
  year={2016}
}



@misc{I2P:2016:transport,
  title = {{I2P} {T}ransport {O}verview},
  howpublished = {\url{https://geti2p.net/en/docs/transport}},
  note = {Last accessed: January 25, 2016}
}

@misc{I2P:2016:stats,
  title = {{I2P} Statistics},
  howpublished = {\url{http://stats.i2p.re/}},
  note = {Last accessed: January 25, 2016}
}

@misc{I2P:2016:peer-profiling,
  title = {{I2P} Peer Profiling and Selection},
  howpublished = {\url{https://geti2p.net/en/docs/how/peer-selection}},
  note = {Last accessed: January 25, 2016}
}

@misc{Shirazi:2016:Survey,
    author = {Fatemeh Shirazi and Milivoj Simeonovski and Muhammad Rizwan Asghar and Claudia Diaz and Michael Backes},
    title = {Survey on {R}outing in {An}onymous {C}ommunication {N}etworks},
    howpublished = {Technical report},
    year = {2016},
    note = {},
}

@misc{AlSabah:2015:Tor-Survey,
    author = {Mashael AlSabah and Ian Goldberg},
    title = {Performance and Security Improvements for {T}or: A Survey},
    howpublished = {Cryptology ePrint Archive, Report 2015/235},
    year = {2015},
}

@misc{Anonymizer:2015,
  title = {Anonymizer},
  howpublished = {\url{https://www.anonymizer.com/}},
  note = {Last accessed: August 05, 2015}
}

@inproceedings{Czumaj:2015:RandomPermutationSwitchingNetworks,
 author = {Czumaj, Artur},
 title = {Random Permutations Using Switching Networks},
 booktitle = {Proceedings of the Forty-seventh Annual ACM Symposium on Theory of Computing},
 series = {STOC '15},
 year = {2015},
 isbn = {978-1-4503-3536-2},
 location = {Portland, Oregon, USA},
 pages = {703--712},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/2746539.2746629},
 doi = {10.1145/2746539.2746629},
 acmid = {2746629},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {Markov chains, random permutations, switching networks},
} 


@misc{JAP:2015,
  title = {{JAP}: Protection of Privacy on the Internet},
  howpublished = {\url{http://anon.inf.tu-dresden.de/index_en.html}},
  note = {Last accessed: August 05, 2015}
}
@article{Klonowski:2015:DynamicsUrns,
  TITLE = {{On the Dynamics of Systems of Urns}},
  AUTHOR = {Klonowski, Marek and Cicho{\'n}, Jacek and Kapelko, Rafal},
  URL = {https://hal.inria.fr/hal-01349058},
  JOURNAL = {{Discrete Mathematics and Theoretical Computer Science}},
  PUBLISHER = {{DMTCS}},
  VOLUME = {17},
  NUMBER = {2},
  PAGES = {235-250},
  YEAR = {2015},
  KEYWORDS = {Coupon Collector Problem ; mix networks ; urn and balls model},
  PDF = {https://hal.inria.fr/hal-01349058/file/2695-9806-1-PB.pdf},
  HAL_ID = {hal-01349058},
  HAL_VERSION = {v1},
}

@Inbook{Movahedi:2015:MPShuffling,
author={Movahedi, Mahnush and Saia, Jared and Zamani, Mahdi},
editor={Scheideler, Christian},
title={Secure Multi-party Shuffling},
bookTitle={Structural Information and Communication Complexity: 22nd International Colloquium, SIROCCO 2015, Montserrat, Spain, July 14-16, 2015. Post-Proceedings},
year={2015},
publisher={Springer International Publishing},
address={Cham},
pages={459--473},
isbn={978-3-319-25258-2},
doi={10.1007/978-3-319-25258-2_32},
url={http://dx.doi.org/10.1007/978-3-319-25258-2_32}
}


@inproceedings{vandenHooff:2015:Vuvuzela,
  author    = {Jelle van den Hooff and
               David Lazar and
               Matei Zaharia and
               Nickolai Zeldovich},
  title     = {Vuvuzela: scalable private messaging resistant to traffic analysis},
  booktitle = {Proceedings of the 25th Symposium on Operating Systems Principles,
               {SOSP} 2015, Monterey, CA, USA, October 4-7, 2015},
  pages     = {137--152},
  year      = {2015},
  crossref  = {DBLP:conf/sosp/2015},
  url       = {http://doi.acm.org/10.1145/2815400.2815417},
  doi       = {10.1145/2815400.2815417},
  timestamp = {Fri, 02 Oct 2015 08:59:57 +0200},
  biburl    = {http://dblp2.uni-trier.de/rec/bib/conf/sosp/HooffLZZ15},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings {Sun:2015:Raptor,
author = {Yixin Sun and Anne Edmundson and Laurent Vanbever and Oscar Li and Jennifer Rexford and Mung Chiang and Prateek Mittal},
title = {{RAPTOR}: Routing Attacks on Privacy in {Tor}},
booktitle = {24th USENIX Security Symposium (USENIX Security 15)},
year = {2015},
month = {Aug},
address = {Washington, D.C.},
url = {https://www.usenix.org/conference/usenixsecurity15/technical-sessions/presentation/sun},
publisher = {USENIX Association},
}

@article{surveyattacks:2015, 
author={Erdin, E. and Zachor, C. and Gunes, M.H.}, 
journal={Communications Surveys Tutorials, IEEE}, 
title={How to Find Hidden Users: A Survey of Attacks on Anonymity Networks}, 
year={2015}, 
volume={PP}, 
number={99}, 
pages={1-1},
}

@inproceedings{Shirazi:2015:MeasuringResilience,
 author = {Shirazi, Fatemeh and Diaz, Claudia and Wright, Joss},
 title = {Towards Measuring Resilience in Anonymous Communication Networks},
 booktitle = {Proceedings of the 14th ACM Workshop on Privacy in the Electronic Society},
 series = {WPES '15},
 year = {2015},
 isbn = {978-1-4503-3820-2},
 location = {Denver, Colorado, USA},
 pages = {95--99},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/2808138.2808152},
 doi = {10.1145/2808138.2808152},
 acmid = {2808152},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {TOR, anonymous communication networks, performance, resilience},
} 


@misc{tormetrics, 
	author = {The {Tor} Project},
	title = {Tor Metrics},
	howpublished = {\url{https://metrics.torproject.org/}},
	note = {Last accessed: August 05, 2015}
}

@misc{torpathspec:2014,
                author = {The {Tor} Project},
                title = {Tor Path Specification},
                howpublished = {\url{https://gitweb.torproject.org/torspec.git/tree/path-spec.txt}},
  note = {Last accessed: August 05, 2015}
}

@inproceedings{Backref:2014,
  author    = {Michael Backes and
               Jeremy Clark and
               Aniket Kate and
               Milivoj Simeonovski and
               Peter Druschel},
  title     = {BackRef: Accountability in Anonymous Communication Networks},
  booktitle = {Applied Cryptography and Network Security - 12th International Conference, {ACNS} 2014, Lausanne, Switzerland, June 10-13, 2014. Proceedings},
  year      = {2014},
  pages     = {380--400}
}

@inproceedings{Cai:2014:Fingerprinting-Defenses,
 author = {Cai, Xiang and Nithyanand, Rishab and Wang, Tao and Johnson, Rob and Goldberg, Ian},
 title = {A Systematic Approach to Developing and Evaluating Website Fingerprinting Defenses},
 booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
 series = {CCS '14},
 year = {2014},
 location = {Scottsdale, Arizona, USA},
 pages = {227--238},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Conrad:2014:I2PTor,
 title = {{Survey on Tor and I2P}},
  author = {Bernd Conrad and Fatemeh Shirazi}, 
  booktitle = {ICIMP}, 
  year = {2014}, 
  month = {July}, 
  pages = {22--28}, 
}

@article{Dingledine:2014:OneGuardTor,
  title={One fast guard for life (or 9 months)},
  author={Dingledine, Roger and Hopper, Nicholas and Kadianakis, George and Mathewson, Nick},
  journal={7th Workshop on Hot Topics in Privacy Enhancing Technologies (HotPETs 2014)},
  year={2014}
}

@inproceedings{Geddes:2014:Imux,
	author    = {John Geddes and
	Rob Jansen and
	Nicholas Hopper},
	title     = {{IMUX:} Managing {Tor} Connections from Two to Infinity, and Beyond},
	booktitle = {Proceedings of the 13th Workshop on Privacy in the Electronic Society,
	{WPES} 2014, Scottsdale, AZ, USA, November 3, 2014},
	pages     = {181--190},
	year      = {2014}
}

@inproceedings{Ghosh:2014:TorPath,
  title={A TorPath to TorCoin: proof-of-bandwidth altcoins for compensating relays},
  author={Ghosh, Mainak and Richardson, Miles and Ford, Bryan and Jansen, Rob},
  booktitle={Workshop on Hot Topics in Privacy Enhancing Technologies (HotPETs)},
  year={2014}
}


@inproceedings{Jansen:2014:Tor-Sniper,
  author    = {Rob Jansen and
               Florian Tschorsch and
               Aaron Johnson and
               Bj{\"{o}}rn Scheuermann},
  title     = {The Sniper Attack: Anonymously Deanonymizing and Disabling the {Tor}
               Network},
  booktitle = {21st Annual Network and Distributed System Security Symposium, {NDSS}
               2014, San Diego, California, USA, February 23-26, 2013},
  year      = {2014},
}

@inproceedings{Jansen:2014:KIST,
	author    = {Rob Jansen and
	John Geddes and
	Chris Wacek and
	Micah Sherr and
	Paul F. Syverson},
	title     = {Never Been {KIST:} {T}or's Congestion Management Blossoms with Kernel-Informed
	Socket Transport},
	booktitle = {Proceedings of the 23rd {USENIX} Security Symposium, San Diego, CA,
	USA, August 20-22, 2014.},
	pages     = {127--142},
	year      = {2014},
}

@inproceedings{Juarez:2014:Fingerprinting,
 author = {Juarez, Marc and Afroz, Sadia and Acar, Gunes and Diaz, Claudia and Greenstadt, Rachel},
 title = {A Critical Evaluation of Website Fingerprinting Attacks},
 booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
 series = {CCS '14},
 year = {2014},
 location = {Scottsdale, Arizona, USA},
 pages = {263--274},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Roos:2014:FN,
  author    = {Stefanie Roos and
               Benjamin Schiller and
               Stefan Hacker and
               Thorsten Strufe},
  title     = {Measuring Freenet in the Wild: Censorship-Resilience under Observation},
  booktitle = {Privacy Enhancing Technologies - 14th International Symposium, {PETS} 2014, Amsterdam, The Netherlands, July 16-18, 2014. Proceedings},
  year      = {2014},
  pages     = {263--282},
}

@incollection{Sankey:2014:Dovetail,
year={2014},
booktitle={Privacy Enhancing Technologies},
volume={8555},
series={Lecture Notes in Computer Science},
editor={De Cristofaro, Emiliano and Murdoch, StevenJ.},
title={Dovetail: Stronger Anonymity in Next-Generation Internet Routing},
publisher={Springer International Publishing},
author={Sankey, Jody and Wright, Matthew},
pages={283-303},
}

@misc{Web:2014:I2P,
  title = {{I2P} Documentation},
  howpublished = {\url{https://geti2p.net/en/docs}},
  note = {Last accessed: August 05, 2014}
}



@misc{Web:2014:garlic-routing,
  title = {Garlic Routing and "Garlic" Terminology},
  howpublished = {\url{https://geti2p.net/en/docs/how/garlic-routing}},
  note = {Last accessed: August 05, 2014}
}

@misc{Web:2014:tunnel-routing, 
  title = {Tunnel Routing},
  howpublished = {\url{https://geti2p.net/en/docs/how/tunnel-routing}},
  note = {Last accessed: August 05, 2014}
}

@inproceedings{AlSabah:2013:PCTCP,
	author    = {Mashael AlSabah and
	Ian Goldberg},
	title     = {{PCTCP:} per-circuit TCP-over-IPsec transport for anonymous communication
	overlay networks},
	booktitle = {2013 {ACM} {SIGSAC} Conference on Computer and Communications Security,
	CCS'13, Berlin, Germany, November 4-8, 2013},
	pages     = {349--360},
	year      = {2013},
}


@INPROCEEDINGS{Backes:2013:AnoA,
author={Backes, M. and Kate, A. and Manoharan, P. and Meiser, S. and Mohammadi, E.}, 
booktitle={Computer Security Foundations Symposium ({CSF}), 2013 IEEE 26th},
title={{AnoA}: A Framework for Analyzing Anonymous Communication Protocols}, 
year={2013}, 
month={June}, 
pages={163-178},
}

@inproceedings{Backes:2014:Mator,
 author = {Backes, Michael and Kate, Aniket and Meiser, Sebastian and Mohammadi, Esfandiar},
 title = {{(Nothing else) MATor(s): Monitoring the Anonymity of {T}or's Path Selection}},
 booktitle = {Proceedings of the 2014 ACM SIGSAC Conference on Computer and Communications Security},
 series = {CCS '14},
 year = {2014},
 location = {Scottsdale, Arizona, USA},
 pages = {513--524},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA}
}

@INPROCEEDINGS{Backes:2014:TUC,
author={Backes, M. and Manoharan, P. and Mohammadi, E.}, 
booktitle={Computer Security Foundations Symposium ({CSF}), 2014 IEEE 27th}, 
title={{TUC}: Time-Sensitive and Modular Analysis of Anonymous Communication}, 
year={2014}, 
month={July}, 
pages={383-397},
}

@incollection{Barbera:2013:CellFlood,
year={2013},
booktitle={Computer Security - {ESORICS} 2013},
volume={8134},
series={Lecture Notes in Computer Science},
editor={Crampton, Jason and Jajodia, Sushil and Mayes, Keith},
title={{CellFlood}: Attacking {Tor} Onion Routers on the Cheap},
publisher={Springer Berlin Heidelberg},
author={Barbera, MarcoValerio and Kemerlis, VasileiosP. and Pappas, Vasilis and Keromytis, AngelosD.},
pages={664-681},
}


@INPROCEEDINGS{Biryukov:2013:HiddenServices,
author={Biryukov, A. and Pustogarov, I. and Weinmann, R.},
booktitle={Security and Privacy ({SP}), 2013 IEEE Symposium on},
title={Trawling for {Tor} Hidden Services: Detection, Measurement, Deanonymization},
year={2013},
month={May},
pages={80-94},
}

@inproceedings{Corrigan-Gibbs:2013,
author = {Henry Corrigan-Gibbs and David Isaac Wolinsky and Bryan Ford},
title = {Proactively Accountable Anonymous Messaging in Verdict},
booktitle = {Presented as part of the 22nd {USENIX Security Symposium (USENIX Security 13)}},
year = {2013},
pages = {147--162},
publisher = {USENIX},
}

@inproceedings{Danezis:2013:MeasuringAnonymity,
  title={Measuring anonymity: a few thoughts and a differentially private bound},
  author={Danezis, George},
  booktitle={Proceedings of the DIMACS Workshop on Measuring Anonymity},
  pages={26},
  year={2013}
}


@inproceedings{Egger:2013:I2P-Practical-attacks,
  title = {Practical Attacks Against the I2P Network}, 
  author = {Christoph Egger and Johannes Schlumberger and Christopher Kruegel and Giovanni
        Vigna}, 
  booktitle = {Proceedings of the 16th International Symposium on Research in Attacks,
        Intrusions and Defenses (RAID 2013)}, 
  year = {2013}, 
  month = {October}, 
  www_pdf_url = {http://wwwcip.informatik.uni-erlangen.de/~spjsschl/i2p.pdf}, 
  www_tags = {selected}, 
  www_section = {Traffic analysis}, 
}

@INPROCEEDINGS{Houmansadr:2013:ParrotisDead,
author={Houmansadr, A. and Brubaker, C. and Shmatikov, V.},
booktitle={Security and Privacy ({SP}), 2013 IEEE Symposium on},
title={The Parrot Is Dead: Observing Unobservable Network Communications},
year={2013},
month={May},
pages={65-79},
}

@inproceedings{Johnson:2013:UGRTor,
 author = {Johnson, Aaron and Wacek, Chris and Jansen, Rob and Sherr, Micah and Syverson, Paul},
 title = {Users Get Routed: Traffic Correlation on Tor by Realistic Adversaries},
 booktitle = {Proceedings of the 2013 ACM SIGSAC Conference on Computer \&\#38; Communications Security},
 series = {CCS '13},
 year = {2013},
 isbn = {978-1-4503-2477-9},
 location = {Berlin, Germany},
 pages = {337--348},
 numpages = {12},
 url = {http://doi.acm.org/10.1145/2508859.2516651},
 doi = {10.1145/2508859.2516651},
 acmid = {2516651},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymity, metrics, onion routing},
} 

[download] 

@inproceedings{Mittal:2013:Pisces,
  title = {Pisces: Anonymous Communication Using Social Networks}, 
  author = {Prateek Mittal and Matthew Wright and Nikita Borisov}, 
  booktitle = {Proceedings of the 20th Annual Network and Distributed System Security
        Symposium ({NDSS} '13)}, 
  year = {2013}, 
  month = {February}, 
  publisher = {The Internet Society 2013}, 
}

@INPROCEEDINGS{Roos:2013:FN,
author={Roos, S. and Strufe, T.}, 
booktitle={INFOCOM, 2013 Proceedings IEEE}, 
title={A contribution to analyzing and enhancing Darknet routing}, 
year={2013}, 
month={April}, 
pages={615-619}, 
}

@inproceedings{Wang:2013:Tor-Fingerprinting,
 author = {Wang, Tao and Goldberg, Ian},
 title = {Improved Website Fingerprinting on {Tor}},
 booktitle = {Proceedings of the 12th {ACM} Workshop on Workshop on Privacy in the Electronic Society},
 series = {{WPES} '13},
 year = {2013},
 location = {Berlin, Germany},
 pages = {201--212},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@INPROCEEDINGS{Akhoondi:2012:LASTor, 
author={Akhoondi, M. and Yu, C. and Madhyastha, H.V.}, 
booktitle={Security and Privacy ({SP}), 2012 IEEE Symposium on}, 
title={LASTor: A Low-Latency AS-Aware {Tor} Client}, 
year={2012}, 
month={May}, 
pages={476-490}, 
}

@inproceedings{AlSabah:2012:Conflux,
	author    = {Mashael AlSabah and
	Kevin S. Bauer and
	Tariq Elahi and
	Ian Goldberg},
	title     = {The Path Less Travelled: Overcoming {T}or's Bottlenecks with Traffic
	Splitting},
	booktitle = {Privacy Enhancing Technologies - 13th International Symposium, {PETS}
	2013, Bloomington, IN, USA, July 10-12, 2013. Proceedings},
	pages     = {143--163},
	year      = {2013},
}

@inproceedings{AlSabah:2012:DiffTor,
	author    = {Mashael AlSabah and
	Kevin S. Bauer and
	Ian Goldberg},
	title     = {Enhancing {T}or's performance using real-time traffic classification},
	booktitle = {the {ACM} Conference on Computer and Communications Security, CCS'12,
	Raleigh, NC, USA, October 16-18, 2012},
	pages     = {73--84},
	year      = {2012}
}

@inproceedings{Backes:2012:Ace,
 author = {Backes, Michael and Kate, Aniket and Mohammadi, Esfandiar},
 title = {Ace: An Efficient Key-exchange Protocol for Onion Routing},
 booktitle = {Proceedings of the 2012 {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '12},
 year = {2012},
 location = {Raleigh, North Carolina, USA},
 pages = {55--64},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@INPROCEEDINGS{Backes:2012:Sec-OR,
author={Backes, M. and Goldberg, I. and Kate, A. and Mohammadi, E.}, 
booktitle={Computer Security Foundations Symposium ({CSF}), 2012 IEEE 25th}, 
title={Provably Secure and Practical Onion Routing}, 
year={2012}, 
month={June}, 
pages={369-385}, 
}

@Inbook{Bayer:2012:EfficentZKProofofShuffle,
author={Bayer, Stephanie
and Groth, Jens},
editor={Pointcheval, David
and Johansson, Thomas},
title={Efficient Zero-Knowledge Argument for Correctness of a Shuffle},
bookTitle={Advances in Cryptology -- EUROCRYPT 2012: 31st Annual International Conference on the Theory and Applications of Cryptographic Techniques, Cambridge, UK, April 15-19, 2012. Proceedings},
year={2012},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={263--280},
isbn={978-3-642-29011-4},
doi={10.1007/978-3-642-29011-4_17},
url={http://dx.doi.org/10.1007/978-3-642-29011-4_17}
}


@article{Danner:2012:DoS-Tor,
 author = {Danner, Norman and Defabbia-Kane, Sam and Krizanc, Danny and Liberatore, Marc},
 title = {Effectiveness and Detection of Denial-of-service Attacks in {Tor}},
 journal = {ACM Trans. Inf. Syst. Secur.},
 issue_date = {November 2012},
 volume = {15},
 number = {3},
 month = {nov},
 year = {2012},
 pages = {11:1--11:25},
 articleno = {11},
 numpages = {25},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@INPROCEEDINGS{Dyer:2012:Traffic-Analysis, 
author={Dyer, K.P. and Coull, S.E. and Ristenpart, T. and Shrimpton, T.}, 
booktitle={Security and Privacy ({SP}), 2012 IEEE Symposium on}, 
title={Peek-a-Boo, I Still See You: Why Efficient Traffic Analysis Countermeasures Fail}, 
year={2012}, 
month={May}, 
pages={332-346}, 
}

@article{Feigenbaum:2012:Routing-Model,
 author = {Feigenbaum, Joan and Johnson, Aaron and Syverson, Paul},
 title = {Probabilistic Analysis of Onion Routing in a Black-box Model},
 journal = {ACM Trans. Inf. Syst. Secur.},
 issue_date = {November 2012},
 volume = {15},
 number = {3},
 month = {November},
 year = {2012},
 pages = {14:1--14:28},
 articleno = {14},
 numpages = {28},
 publisher = {ACM},
 address = {New York, NY, USA},
}


@incollection{Gilad:2012:Traffic-Analysis,
year={2012},
booktitle={Privacy Enhancing Technologies},
volume={7384},
series={Lecture Notes in Computer Science},
editor={Fischer-H{\"{u}}bner, Simone and Wright, Matthew},
title={Spying in the Dark: {TCP} and {Tor} Traffic Analysis},
publisher={Springer Berlin Heidelberg},
author={Gilad, Yossi and Herzberg, Amir},
pages={100-119},
}

@Inbook{Goodrich:2012:AnonymousCardShuffling,
author={Goodrich, Michael T.
and Mitzenmacher, Michael},
editor={Czumaj, Artur
and Mehlhorn, Kurt
and Pitts, Andrew
and Wattenhofer, Roger},
title={Anonymous Card Shuffling and Its Applications to Parallel Mixnets},
bookTitle={Automata, Languages, and Programming: 39th International Colloquium, ICALP 2012, Warwick, UK, July 9-13, 2012, Proceedings, Part II},
year={2012},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={549--560},
isbn={978-3-642-31585-5},
doi={10.1007/978-3-642-31585-5_49},
url={http://dx.doi.org/10.1007/978-3-642-31585-5_49}
}


@inproceedings{Gopal:2012:Torchestra,
 author = {Gopal, Deepika and Heninger, Nadia},
 title = {Torchestra: Reducing Interactive Traffic Delays over {Tor}},
 booktitle = {Proceedings of the 2012 {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '12},
 year = {2012},
 location = {Raleigh, North Carolina, USA},
 pages = {31--42},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Jansen:2012:ThrottlingBWTor,
	author    = {Rob Jansen and
	Paul F. Syverson and
	Nicholas Hopper},
	title     = {Throttling {Tor} Bandwidth Parasites},
	booktitle = {Proceedings of the 21th {USENIX} Security Symposium, Bellevue, WA,
	USA, August 8-10, 2012},
	pages     = {349--363},
	year      = {2012},
}

@inproceedings{MohajeriMoghaddam:2012:SkypeMorph,
 author = {Mohajeri Moghaddam, Hooman and Li, Baiyu and Derakhshani, Mohammad and Goldberg, Ian},
 title = {{SkypeMorph}: Protocol Obfuscation for {Tor} Bridges},
 booktitle = {Proceedings of the 2012 ACM Conference on Computer and Communications Security},
 series = {{CCS} '12},
 year = {2012},
 pages = {97--108},
 numpages = {12},
 publisher = {ACM},
}

@inproceedings{Panchenko:2012:ImprovingTorPerformance,
	author    = {Andriy Panchenko and
	Fabian Lanze and
	Thomas Engel},
	title     = {Improving performance and anonymity in the {Tor} network},
	booktitle = {31st {IEEE} International Performance Computing and Communications
	Conference, {IPCCC} 2012, Austin, TX, USA, December 1-3, 2012},
	pages     = {1--10},
	year      = {2012}
}

@incollection{Timpanaro:2012:I2P,
year={2012},
booktitle={Traffic Monitoring and Analysis},
volume={7189},
series={Lecture Notes in Computer Science},
editor={Pescap{\`{e}}, Antonio and Salgarelli, Luca and Dimitropoulos, Xenofontas},
title={{I2P}'s Usage Characterization},
publisher={Springer Berlin Heidelberg},
author={Timpanaro, Juan Pablo and Chrisment, Isabelle and Festor, Olivier},
pages={48-51},
}

@article{Wang:2012:Octopus,
  author    = {Qiyan Wang and
               Nikita Borisov},
  title     = {Octopus: {A} Secure and Anonymous {DHT} Lookup},
  journal   = {CoRR},
  volume    = {abs/1203.2668},
  year      = {2012},
  url       = {http://arxiv.org/abs/1203.2668},
  timestamp = {Wed, 10 Oct 2012 21:28:49 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/journals/corr/abs-1203-2668},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@incollection{Wang:2012:Tor-CongestionAware,
year={2012},
booktitle={Financial Cryptography and Data Security},
volume={7397},
series={Lecture Notes in Computer Science},
editor={Keromytis, AngelosD.},
title={Congestion-Aware Path Selection for {Tor}},
publisher={Springer Berlin Heidelberg},
author={Wang, Tao and Bauer, Kevin and Forero, Clara and Goldberg, Ian},
pages={98-113},
}

@inproceedings{Weinberg:2012:StegoTorus,
 author = {Weinberg, Zachary and Wang, Jeffrey and Yegneswaran, Vinod and Briesemeister, Linda and Cheung, Steven and Wang, Frank and Boneh, Dan},
 title = {StegoTorus: A Camouflage Proxy for the {Tor} Anonymity System},
 booktitle = {Proceedings of the 2012 {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '12},
 year = {2012},
 location = {Raleigh, North Carolina, USA},
 pages = {109--120},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Wolinsky:2012:Dissent,
 author = {Wolinsky, David Isaac and Corrigan-Gibbs, Henry and Ford, Bryan and Johnson, Aaron},
 title = {Dissent in Numbers: Making Strong Anonymity Scale},
 booktitle = {Proceedings of the 10th USENIX Conference on Operating Systems Design and Implementation},
 series = {{OSDI} '12},
 year = {2012},
 pages = {179--192},
 numpages = {14},
 publisher = {USENIX Association},
}

@inproceedings{Wolinsky:2012:Dissent-anytrust,
  title={Scalable anonymous group communication in the anytrust model},
  author={Wolinsky, David Isaac and Corrigan-Gibbs, Henry and Ford, Bryan and Johnson, Aaron},
  booktitle={European Workshop on System Security ({EuroSec})},
  volume={4},
  year={2012}
}

@incollection{Alsabah:2011:DefenestraTor,
year={2011},
booktitle={Privacy Enhancing Technologies},
volume={6794},
series={Lecture Notes in Computer Science},
editor={Fischer-H{\"{u}}bner, Simone and Hopper, Nicholas},
title={DefenestraTor: Throwing Out Windows in {Tor}},
publisher={Springer Berlin Heidelberg},
author={AlSabah, Mashael and Bauer, Kevin and Goldberg, Ian and Grunwald, Dirk and McCoy, Damon and Savage, Stefan and Voelker, GeoffreyM.},
pages={134-154},
}

@INPROCEEDINGS{Evans:2011:R5N, 
author={Evans, N.S. and Grothoff, C.}, 
booktitle={Network and System Security ({NSS}), 2011 5th International Conference on}, 
title={{R5N}: Randomized recursive routing for restricted-route networks}, 
year={2011}, 
month={September}, 
pages={316-321},
}

@INPROCEEDINGS{Hsiao:2011:LAP, 
author={Hsu-Chun Hsiao and Kim, T.H.-J. and Perrig, A. and Yamada, A. and Nelson, S.C. and Gruteser, M. and Wei Meng}, 
booktitle={Security and Privacy ({SP}), 2012 IEEE Symposium on}, 
title={{LAP}: Lightweight Anonymity and Privacy}, 
year={2012}, 
month={May}, 
pages={506-520}, 
}

@inproceedings{Mittal:2011:PIR-Tor,
 author = {Mittal, Prateek and Olumofin, Femi and Troncoso, Carmela and Borisov, Nikita and Goldberg, Ian},
 title = {{PIR-Tor}: Scalable Anonymous Communication Using Private Information Retrieval},
 booktitle = {Proceedings of the 20th {USENIX} Conference on Security},
 series = {{SEC} '11},
 year = {2011},
 location = {San Francisco, CA},
 pages = {31--31},
 numpages = {1},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
}

@inproceedings{Mittal:2011:Tor-Attack,
 author = {Mittal, Prateek and Khurshid, Ahmed and Juen, Joshua and Caesar, Matthew and Borisov, Nikita},
 title = {Stealthy Traffic Analysis of Low-latency Anonymous Communication Using Throughput Fingerprinting},
 booktitle = {Proceedings of the 18th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '11},
 year = {2011},
 location = {Chicago, Illinois, USA},
 pages = {215--226},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Panchenko:2011:OR-Fingerprinting,
 author = {Panchenko, Andriy and Niessen, Lukas and Zinnen, Andreas and Engel, Thomas},
 title = {Website Fingerprinting in Onion Routing Based Anonymization Networks},
 booktitle = {Proceedings of the 10th Annual {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '11},
 year = {2011},
 location = {Chicago, Illinois, USA},
 pages = {103--114},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Moore:2011:RateLimitingTor,
	author    = {W. Brad Moore and
	Chris Wacek and
	Micah Sherr},
	title     = {Exploring the potential benefits of expanded rate limiting in {T}or:
	slow and steady wins the race with Tortoise},
	booktitle = {Twenty-Seventh Annual Computer Security Applications Conference, {ACSAC} 2011, Orlando, FL, USA, 5-9 December 2011},
	pages     = {207--216},
	year      = {2011}
}

@ARTICLE{Snader:2011:Tor-tuneup, 
author={Snader, R. and Borisov, N.}, 
journal={Dependable and Secure Computing, {IEEE} Transactions on}, 
title={Improving Security and Performance in the {Tor} Network through Tunable Path Selection}, 
year={2011}, 
month={September}, 
volume={8}, 
number={5}, 
pages={728-741}, 
}

@techreport{Timpanaro:2011:MonitoringI2P,
  TITLE = {{Monitoring the {I2P} network}},
  AUTHOR = {Timpanaro, Juan Pablo and Isabelle, Chrisment and Olivier, Festor},
  URL = {https://hal.inria.fr/hal-00653136},
  YEAR = {2011},
  MONTH = {October},
}

@Inbook{Beimel:2010:CoinToss,
author={Beimel, Amos and Omri, Eran and Orlov, Ilan},
editor={Rabin, Tal},
title={Protocols for Multiparty Coin Toss with Dishonest Majority},
bookTitle={Advances in Cryptology -- CRYPTO 2010: 30th Annual Cryptology Conference, Santa Barbara, CA, USA, August 15-19, 2010. Proceedings},
year={2010},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={538--557},
isbn={978-3-642-14623-7},
doi={10.1007/978-3-642-14623-7_29},
url={http://dx.doi.org/10.1007/978-3-642-14623-7_29}
}

@incollection{Chakravarty:2010:TA-BW,
year={2010},
booktitle={Computer Security - {ESORICS} 2010},
volume={6345},
series={Lecture Notes in Computer Science},
editor={Gritzalis, Dimitris and Preneel, Bart and Theoharidou, Marianthi},
title={Traffic Analysis against Low-Latency Anonymity Networks Using Available Bandwidth Estimation},
publisher={Springer Berlin Heidelberg},
author={Chakravarty, Sambuddho and Stavrou, Angelos and Keromytis, AngelosD.},
pages={249-267},
}

@article{Clarke:2010:FN,
  title={Private communication through a network of trusted connections: The dark freenet},
  author={Clarke, Ian and Sandberg, Oskar and Toseland, Matthew and Verendel, Vilhelm},
  journal={Network},
  year={2010}
}

@inproceedings{Corrigan-Gibbs:2010:Dissent,
 author = {Corrigan-Gibbs, Henry and Ford, Bryan},
 title = {Dissent: Accountable Anonymous Group Messaging},
 booktitle = {Proceedings of the 17th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '10},
 year = {2010},
 pages = {340--350},
 numpages = {11}
}


@inproceedings{Diaz:2010:TopologyComparisonMixnets,
 author = {Diaz, Claudia and Murdoch, Steven J. and Troncoso, Carmela},
 title = {Impact of Network Topology on Anonymity and Overhead in Low-latency Anonymity Networks},
 booktitle = {Proceedings of the 10th International Conference on Privacy Enhancing Technologies},
 series = {PETS'10},
 year = {2010},
 isbn = {3-642-14526-4, 978-3-642-14526-1},
 location = {Berlin, Germany},
 pages = {184--201},
 numpages = {18},
 url = {http://dl.acm.org/citation.cfm?id=1881151.1881162},
 acmid = {1881162},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@inproceedings{Gong:2010:Traffic-Analysis,
 author = {Gong, Xun and Kiyavash, Negar and Borisov, Nikita},
 title = {Fingerprinting Websites Using Remote Traffic Analysis},
 booktitle = {Proceedings of the 17th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '10},
 year = {2010},
 location = {Chicago, Illinois, USA},
 pages = {684--686},
 numpages = {3},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{Hopper:2010:Leakage,
 author = {Hopper, Nicholas and Vasserman, Eugene Y. and Chan-TIN, Eric},
 title = {How Much Anonymity Does Network Latency Leak?},
 journal = {ACM Trans. Inf. Syst. Secur.},
 volume = {13},
 number = {2},
 month = {March},
 year = {2010},
 pages = {13:1--13:28},
 articleno = {13},
 numpages = {28},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@Inbook{Juels:2010:JCJ,
author={Juels, Ari and Catalano, Dario and Jakobsson, Markus},
editor={Chaum, David and Jakobsson, Markus and Rivest, Ronald L. and Ryan, Peter Y. A. and Benaloh, Josh and Kutylowski, Miroslaw and Adida, Ben},
title={Coercion-Resistant Electronic Elections},
bookTitle={Towards Trustworthy Elections: New Directions in Electronic Voting},
year={2010},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={37--63},
isbn={978-3-642-12980-3},
doi={10.1007/978-3-642-12980-3_2},
url={http://dx.doi.org/10.1007/978-3-642-12980-3_2}
}


@article{Kate:2010:OR-Pairing,
 author = {Kate, Aniket and Zaverucha, Greg M. and Goldberg, Ian},
 title = {Pairing-Based Onion Routing with Improved Forward Secrecy},
 journal = {ACM Trans. Inf. Syst. Secur.},
 issue_date = {December 2010},
 volume = {13},
 number = {4},
 month = {December},
 year = {2010},
 pages = {29:1--29:32},
 articleno = {29},
 numpages = {32},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@misc{Pfitzmann:2010:ATerminology, 
	author = {Andreas Pfitzmann and Marit Hansen},
	title = {A terminology for talking about privacy by data minimization: 
		Anonymity, Unlinkability, Undetectability, Unobservability, 
		Pseudonymity, and Identity Management},
	month = {August},
	year = {2010},
	howpublished = {\url{http://dud.inf.tu-dresden.de/literatur/Anon_Terminology_v0.34.pdf}},
	note = {Last accessed: August 05, 2015}
}

@article{Ren:2010:Survey,
  title = {Survey on anonymous communications in computer networks},
  author = {Jian Ren and Jie Wu},
  journal = {Computer Communications},
  volume={33},
  number={4},
  pages={420--431},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{Tang:2010:Tor-CircuitScheduling,
 author = {Tang, Can and Goldberg, Ian},
 title = {An Improved Algorithm for {Tor} Circuit Scheduling},
 booktitle = {Proceedings of the 17th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '10},
 year = {2010},
 location = {Chicago, Illinois, USA},
 pages = {329--339},
 numpages = {11},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{Zhu:2010:CorrelationAnon,
  author    = {Ye Zhu and
               Xinwen Fu and
               Bryan Graham and
               Riccardo Bettati and
               Wei Zhao},
  title     = {Correlation-Based Traffic Analysis Attacks on Anonymity Networks},
  journal   = {{IEEE} Trans. Parallel Distrib. Syst.},
  volume    = {21},
  number    = {7},
  pages     = {954--967},
  year      = {2010}
}

@incollection{Danezis:2009:Survey,
  title = {{Systems for Anonymous Communication}}, 
  author = {George Danezis and Claudia Diaz and Paul F. Syverson}, 
  booktitle = {CRC Handbook of Financial Cryptography and Security}, 
  volume = {}, 
  year = {2010}, 
  month = {August}, 
  pages = {341--390}, 
  editor = {B. Rosenberg and D. Stinson}, 
  publisher = {Chapman \& Hall}, 
  series = {{CRC} Cryptography and Network Security Series},
  www_pdf_url = {https://www.cosic.esat.kuleuven.be/publications/article-1335.pdf}, 
}

@incollection{Danezis:2009:WisdomCrowds,
year={2009},
booktitle={Computer Security – {ESORICS} 2009},
volume={5789},
series={Lecture Notes in Computer Science},
editor={Backes, Michael and Ning, Peng},
title={The Wisdom of Crowds: Attacks and Optimal Constructions},
publisher={Springer Berlin Heidelberg},
author={Danezis, George and Diaz, Claudia and Käsper, Emilia and Troncoso, Carmela},
pages={406-423},
}

@Inbook{Danezis:2009:Vida,
author={Danezis, George and Troncoso, Carmela},
editor={Goldberg, Ian and Atallah, Mikhail J.},
title={Vida: How to Use Bayesian Inference to De-anonymize Persistent Communications},
bookTitle={Privacy Enhancing Technologies: 9th International Symposium, PETS 2009, Seattle, WA, USA, August 5-7, 2009. Proceedings},
year={2009},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={56--72},
isbn={978-3-642-03168-7},
doi={10.1007/978-3-642-03168-7_4},
url={http://dx.doi.org/10.1007/978-3-642-03168-7_4}
}


@techreport{Dingledine:2009:TorTechReport,
  author = {Roger Dingledine and Steven J. Murdoch},
  title = {Performance Improvements on {Tor} or, Why {Tor} is slow and what we're going to do about it},
  institution = {The {Tor} Project},
  year = {2009},
  month = {November},
  url = {https://research.torproject.org/techreports/performance-2009-11-09.pdf}
}

@inproceedings{Edman:2009:Tor-AS-Aware,
 author = {Edman, Matthew and Syverson, Paul},
 title = {As-awareness in {Tor} Path Selection},
 booktitle = {Proceedings of the 16th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '09},
 year = {2009},
 location = {Chicago, Illinois, USA},
 pages = {380--389},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{Edman:2009:Survey,
 author = {Edman, Matthew and Yener, B\"{u}lent},
 title = {On Anonymity in an Electronic Society: A Survey of Anonymous Communication Systems},
 journal = {ACM Computing Surveys (CSUR)},
 volume = {42},
 number = {1},
 month = {December},
 year = {2009},
 pages = {5:1--5:35},
 articleno = {5},
 numpages = {35},
 publisher = {ACM},
}

@inproceedings {Evans:2009:Tor-Congestion-Attacks,
	title = {A Practical Congestion Attack on {Tor} Using Long Paths},
	booktitle = {Presented as part of the 18th {USENIX Security Symposium (USENIX Security 09)}},
	year = {2009},
	address = {Montreal, Canada},
	url = {https://www.usenix.org/node/},
	authors={Nathan S. Evans, Roger Dingledine, Christian Grothoff},
	publisher = {USENIX},
}

@inproceedings{Johnson:2009:OR-Trust,
  author    = {Aaron Johnson and
               Paul F. Syverson},
  title     = {More Anonymous Onion Routing Through Trust},
  booktitle = {Proceedings of the 22nd {IEEE} Computer Security Foundations Symposium,
               {CSF} 2009, Port Jefferson, New York, USA, July 8-10, 2009},
  pages     = {3--12},
  year      = {2009},
  crossref  = {DBLP:conf/csfw/2009},
}


@inproceedings{Kate:2009:AsyncDistrKeyGen,
  author    = {Aniket Kate and
               Ian Goldberg},
  title     = {Distributed Key Generation for the Internet},
  booktitle = {29th {IEEE} International Conference on Distributed Computing Systems
               {(ICDCS} 2009), 22-26 June 2009, Montreal, Qu{\'{e}}bec, Canada},
  pages     = {119--128},
  year      = {2009},
  crossref  = {DBLP:conf/icdcs/2009},
  url       = {http://dx.doi.org/10.1109/ICDCS.2009.21},
  doi       = {10.1109/ICDCS.2009.21},
  timestamp = {Thu, 11 Dec 2014 17:34:06 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/icdcs/KateG09},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@proceedings{DBLP:conf/csfw/2009,
  title     = {Proceedings of the 22nd {IEEE} Computer Security Foundations Symposium,
               {CSF} 2009, Port Jefferson, New York, USA, July 8-10, 2009},
  publisher = {{IEEE} Computer Society},
  year      = {2009},
}

@inproceedings{McLachlan:2009:Torsk,
 author = {McLachlan, Jon and Tran, Andrew and Hopper, Nicholas and Kim, Yongdae},
 title = {Scalable Onion Routing with {Torsk}},
 booktitle = {Proceedings of the 16th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '09},
 year = {2009},
 location = {Chicago, Illinois, USA},
 pages = {590--599},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Mittal:2009:ShadowWalker,
 author = {Mittal, Prateek and Borisov, Nikita},
 title = {{ShadowWalker}: Peer-to-peer Anonymous Communication Using Redundant Structured Topologies},
 booktitle = {Proceedings of the 16th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '09},
 year = {2009},
 pages = {161--172},
 numpages = {12},
 publisher = {ACM},
}

@inproceedings{Panchenko:2009:NISAN,
	author    = {Andriy Panchenko and
	Stefan Richter and
	Arne Rache},
	title     = {{NISAN:} network information service for anonymization networks},
	booktitle = {Proceedings of the 2009 {ACM} Conference on Computer and Communications
	Security, {CCS} 2009, Chicago, Illinois, USA, November 9-13, 2009},
	pages     = {141--150},
	year      = {2009}
}

@inproceedings{Schimmer:2009:I2P, 
 title = {Peer Profiling and Selection in the {I2P} Anonymous Network}, 
  author = {Lars Schimmer}, 
  booktitle = {Proceedings of {PET-CON} 2009.1}, 
  year = {2009}, 
  month = {March}, 
  pages = {59--70}, 
}

@inproceedings{Sherr:2009:Tor-Link-BasedSelection,
  title = {Scalable Link-Based Relay Selection for Anonymous Routing}, 
  author = {Micah Sherr and Matt Blaze and Boon Thau Loo}, 
  booktitle = {Proceedings of Privacy Enhancing Technologies, 9th International Symposium
        ({PETS} 2009)}, 
  volume = {5672}, 
  year = {2009}, 
  month = {August}, 
  pages = {73--93}, 
  editor = {Ian Goldberg and Mikhail J. Atallah}, 
  publisher = {Springer}, 
  series = {Lecture Notes in Computer Science}, 
  www_section = {Anonymous communication,Tor Performance}, 
  www_pdf_url = {http://micah.cis.upenn.edu/papers/pets09.pdf}, 
}

@inproceedings{Syverson:2009:NotEntropist,
  title={Why I’m not an entropist},
  author={Syverson, Paul},
  booktitle={International Workshop on Security Protocols},
  pages={213--230},
  year={2009},
  organization={Springer Berlin Heidelberg}
}


@inproceedings{Tran:2009:Sybil,
  title={Sybil-Resilient Online Content Voting.},
  author={Tran, Dinh Nguyen and Min, Bonan and Li, Jinyang and Subramanian, Lakshminarayanan},
  booktitle={{NSDI}},
  volume={9},
  number={1},
  pages={15--28},
  year={2009}
}

@inproceedings{Troncoso:2009:Bayesian,
 author = {Troncoso, Carmela and Danezis, George},
 title = {The Bayesian Traffic Analysis of Mix Networks},
 booktitle = {Proceedings of the 16th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '09},
 year = {2009},
 location = {Chicago, Illinois, USA},
 pages = {369--379},
 numpages = {11},
 publisher = {ACM},
 address = {New York, NY, USA},
}


@inproceedings{Vasserman:2009:Membership,
 author = {Vasserman, Eugene and Jansen, Rob and Tyra, James and Hopper, Nicholas and Kim, Yongdae},
 title = {Membership-concealing Overlay Networks},
 booktitle = {Proceedings of the 16th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '09},
 year = {2009},
 pages = {390--399},
 numpages = {10},
 publisher = {ACM},
}

@inproceedings{Wikstrom:2009:CommitmentProofofShuffle,
  author    = {Douglas Wikstr{\"{o}}m},
  title     = {A Commitment-Consistent Proof of a Shuffle},
  booktitle = {Information Security and Privacy, 14th Australasian Conference, {ACISP}
               2009, Brisbane, Australia, July 1-3, 2009, Proceedings},
  pages     = {407--421},
  year      = {2009},
  url       = {http://dx.doi.org/10.1007/978-3-642-02620-1_28},
  doi       = {10.1007/978-3-642-02620-1_28},
  timestamp = {Wed, 24 Jun 2009 11:57:28 +0200},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/acisp/Wikstrom09},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}

@inproceedings{Adida:2008:Helios,
 author = {Adida, Ben},
 title = {Helios: Web-based Open-audit Voting},
 booktitle = {Proceedings of the 17th Conference on Security Symposium},
 series = {SS'08},
 year = {2008},
 location = {San Jose, CA},
 pages = {335--348},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=1496711.1496734},
 acmid = {1496734},
 publisher = {USENIX Association},
 address = {Berkeley, CA, USA},
} 

@inproceedings{Clarkson:2008:Civitas,
 author = {Clarkson, Michael R. and Chong, Stephen and Myers, Andrew C.},
 title = {Civitas: Toward a Secure Voting System},
 booktitle = {Proceedings of the 2008 IEEE Symposium on Security and Privacy},
 series = {SP '08},
 year = {2008},
 isbn = {978-0-7695-3168-7},
 pages = {354--368},
 numpages = {15},
 url = {http://dx.doi.org/10.1109/SP.2008.32},
 doi = {10.1109/SP.2008.32},
 acmid = {1398035},
 publisher = {IEEE Computer Society},
 address = {Washington, DC, USA},
 keywords = {Electronic voting, verifiable elections, coercion resistance, voter registration, cryptographic protocols, secure bulletin boards},
} 

@inproceedings{Danezis:2008:RouteBridgingAttacks,
 author = {Danezis, George and Syverson, Paul},
 title = {Bridging and Fingerprinting: Epistemic Attacks on Route Selection},
 booktitle = {Proceedings of the 8th International Symposium on Privacy Enhancing Technologies},
 series = {{PETS} '08},
 year = {2008},
 location = {Leuven, Belgium},
 pages = {151--166},
 numpages = {16},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
}


@techreport{Danezis:2008:Survey,
  title={A survey of anonymous communication channels},
  author={Danezis, George and D{\'{\i}}az, Claudia},
  year={2008},
  institution={Microsoft Research},
}


@incollection{Hevia:2008:Indistinguishability,
year={2008},
booktitle={Privacy Enhancing Technologies},
volume={5134},
series={Lecture Notes in Computer Science},
editor={Borisov, Nikita and Goldberg, Ian},
title={An Indistinguishability-Based Characterization of Anonymous Channels},
publisher={Springer Berlin Heidelberg},
author={Hevia, Alejandro and Micciancio, Daniele},
pages={24-43},
}


@INPROCEEDINGS{Haifeng:2008:Sybil, 
author={Haifeng Yu and Gibbons, P.B. and Kaminsky, M. and Feng Xiao}, 
booktitle={Security and Privacy, 2008. {SP} 2008. {IEEE} Symposium on}, 
title={{SybilLimit}: A Near-Optimal Social Network Defense against Sybil Attacks}, 
year={2008}, 
month={May}, 
pages={3-17},
}

@inproceedings{Kelly:2008:AnonymityMetricSurvey,
 author = {Kelly, Douglas J. and Raines, Richard A. and Grimaila, Michael R. and Baldwin, Rusty O. and Mullins, Barry E.},
 title = {A Survey of State-of-the-art in Anonymity Metrics},
 booktitle = {Proceedings of the 1st ACM Workshop on Network Data Anonymization},
 series = {NDA '08},
 year = {2008},
 isbn = {978-1-60558-301-3},
 location = {Alexandria, Virginia, USA},
 pages = {31--40},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/1456441.1456453},
 doi = {10.1145/1456441.1456453},
 acmid = {1456453},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymity, communication networks, metrics, network data, privacy},
} 



@incollection{Troncoso:2008:Disclosure,
year={2008},
booktitle={Privacy Enhancing Technologies},
volume={5134},
series={Lecture Notes in Computer Science},
editor={Borisov, Nikita and Goldberg, Ian},
title={Perfect Matching Disclosure Attacks},
publisher={Springer Berlin Heidelberg},
author={Troncoso, Carmela and Gierlichs, Benedikt and Preneel, Bart and Verbauwhede, Ingrid},
pages={2-23},
}

@inproceedings{Abbott:2007:Tor-BrowserAttack,
  title = {Browser-Based Attacks on {Tor}}, 
  author = {Tim Abbott and Katherine J. Lai and Michael R. Lieberman and Eric C. Price}, 
  booktitle = {Proceedings of the Seventh Workshop on Privacy Enhancing Technologies ({PET} 2007)}, 
  year = {2007}, 
  month = {June}, 
  location = {Ottawa, Canada}, 
  editor = {Nikita Borisov and Philippe Golle}, 
  publisher = {Springer}, 
  www_pdf_url = {http://petworkshop.org/2007/papers/PET2007_preproc_Browser_based.pdf}, 
}

@inproceedings{Bauer:2007:Attack,
 author = {Bauer, Kevin and McCoy, Damon and Grunwald, Dirk and Kohno, Tadayoshi and Sicker, Douglas},
 title = {Low-resource Routing Attacks Against {Tor}},
 booktitle = {Proceedings of the 2007 {ACM} Workshop on Privacy in Electronic Society},
 series = {{WPES} '07},
 year = {2007},
 location = {Alexandria, Virginia, USA},
 pages = {11--20},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@article{Danezis:2007:Mix-Break,
year={2007},
journal={International Journal of Information Security},
volume={6},
number={6},
title={Breaking four mix-related schemes based on Universal Re-encryption},
publisher={Springer-Verlag},
author={Danezis, George},
pages={393-402},
}

@incollection{Danezis:2007:2-Stat,
year={2007},
booktitle={Privacy Enhancing Technologies},
volume={4776},
series={Lecture Notes in Computer Science},
editor={Borisov, Nikita and Golle, Philippe},
title={Two-Sided Statistical Disclosure Attack},
publisher={Springer Berlin Heidelberg},
author={Danezis, George and D{\'{\i}}az, Claudia and Troncoso, Carmela},
pages={30-44},
}

@inproceedings{Borisov:2007:SDOS,
	author    = {Nikita Borisov and
	George Danezis and
	Prateek Mittal and
	Parisa Tabriz},
	title     = {Denial of service or denial of security?},
	booktitle = {Proceedings of the 2007 {ACM} Conference on Computer and Communications
	Security, {CCS} 2007, Alexandria, Virginia, USA, October 28-31, 2007},
	pages     = {92--102},
	year      = {2007}
}

@incollection{diaz:2007:accountable,
  title={Accountable anonymous communication},
  author={D{\'{\i}}az, Claudia and Preneel, Bart},
  booktitle={Security, Privacy, and Trust in Modern Data Management},
  pages={239--253},
  year={2007},
  publisher={Springer}
}

@INPROCEEDINGS{Edman:2007:Combinatorial,
author={Edman, M. and Sivrikaya, F. and Yener, B.}, 
booktitle={Intelligence and Security Informatics, 2007 IEEE}, 
title={A Combinatorial Approach to Measuring Anonymity}, 
year={2007}, 
month={May}, 
pages={356-363},
}

@article{Gennaro:2007:DistrKeyGen,
author={Gennaro, Rosario and Jarecki, Stanislaw and Krawczyk, Hugo and Rabin, Tal},
title={Secure Distributed Key Generation for Discrete-Log Based Cryptosystems},
journal={Journal of Cryptology},
year={2007},
volume={20},
number={1},
pages={51--83},
abstract={A Distributed Key Generation (DKG) protocol is an essential component of threshold cryptosystems required to initialize the cryptosystem securely and generate its private and public keys. 
In the case of discrete-log-based (dlog-based) threshold signature schemes (ElGamal and its derivatives), the DKG protocol is further used in the distributed signature generation phase to generate one-time signature randomizers (r = gk). 
In this paper we show that a widely used dlog-based DKG protocol suggested by Pedersen does not guarantee a uniformly random distribution of generated keys: 
we describe an efficient  active attacker controlling a small number of parties which successfully biases the values of the generated keys away from uniform. 
We then present a new DKG protocol for the setting of dlog-based cryptosystems which we prove to satisfy the security requirements from DKG protocols and, in particular, it ensures a uniform  distribution of the generated keys. 
The new protocol can be used as a secure replacement for the many applications of Pedersen's protocol. 
Motivated by the fact that the new DKG protocol incurs additional communication cost relative to Pedersen's original protocol, we investigate whether the latter can be used in specific applications which require relaxed security properties from the DKG protocol. 
We answer this question affirmatively by showing that Pedersen's protocol suffices for the secure implementation of certain threshold cryptosystems whose security can be reduced to the hardness of the discrete logarithm problem. 
In particular, we show Pedersen's DKG to be sufficient for the construction of a threshold Schnorr signature scheme. 
Finally, we observe an interesting trade-off between security (reductions), computation, and communication that arises when comparing Pedersen's DKG protocol with ours.},
issn={1432-1378},
doi={10.1007/s00145-006-0347-3},
url={http://dx.doi.org/10.1007/s00145-006-0347-3}
}

@article{Haeberlen:2007:PeerReview,
 author = {Haeberlen, Andreas and Kouznetsov, Petr and Druschel, Peter},
 title = {{PeerReview}: Practical Accountability for Distributed Systems},
 journal = {SIGOPS Oper. Syst. Rev.},
 issue_date = {December 2007},
 volume = {41},
 number = {6},
 month = {October},
 year = {2007},
 pages = {175--188},
 numpages = {14},
 publisher = {ACM},
}

@incollection{Murdoch:2007:Traffic-Analysis,
year={2007},
booktitle={Privacy Enhancing Technologies},
volume={4776},
series={Lecture Notes in Computer Science},
editor={Borisov, Nikita and Golle, Philippe},
title={Sampled Traffic Analysis by Internet-Exchange-Level Adversaries},
author={Murdoch, StevenJ. and Zielinski, Piotr},
pages={167-183},
}

@incollection{Okamoto:2007:Ring,
year={2007},
booktitle={Public Key Cryptography - {PKC} 2007},
volume={4450},
series={Lecture Notes in Computer Science},
editor={Okamoto, Tatsuaki and Wang, Xiaoyun},
title={Traceable Ring Signature},
publisher={Springer Berlin Heidelberg},
author={Fujisaki, Eiichiro and Suzuki, Koutarou},
pages={181-200},
}

@inproceedings{Steiner:2007:Kad,
 author = {Steiner, Moritz and En-Najjary, Taoufik and Biersack, Ernst W.},
 title = {A Global View of Kad},
 booktitle = {Proceedings of the 7th {ACM SIGCOMM} Conference on Internet Measurement},
 series = {{IMC} '07},
 year = {2007},
 location = {San Diego, California, USA},
 pages = {117--122},
 numpages = {6},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Abbott:2007:Tor-BrowserAttack,
title = {Browser-Based Attacks on {Tor}}, 
author = {Tim Abbott and Katherine J. Lai and Michael R. Lieberman and Eric C. Price}, 
booktitle = {Proceedings of the Seventh Workshop on Privacy Enhancing Technologies ({PET} 2007)}, 
year = {2007}, 
month = {June}, 
location = {Ottawa, Canada}, 
editor = {Nikita Borisov and Philippe Golle}, 
publisher = {Springer}
}

@incollection{Feigenbaum:2007:OR-Model,
year={2007},
booktitle={Financial Cryptography and Data Security},
volume={4886},
series={Lecture Notes in Computer Science},
editor={Dietrich, Sven and Dhamija, Rachna},
title={A Model of Onion Routing with Provable Anonymity},
publisher={Springer Berlin Heidelberg},
author={Feigenbaum, Joan and Johnson, Aaron and Syverson, Paul},
pages={57-71},
}

@inproceedings{Brickell:2006:Mining,
 author = {Brickell, Justin and Shmatikov, Vitaly},
 title = {Efficient Anonymity-preserving Data Collection},
 booktitle = {Proceedings of the 12th {ACM SIGKDD} International Conference on Knowledge Discovery and Data Mining},
 series = {{KDD} '06},
 year = {2006},
 pages = {76--85},
 numpages = {10},
 publisher = {ACM},
}

@inproceedings{Danezis:2006:Fingerprinting,
  title={Route fingerprinting in anonymous communications},
  author={Danezis, George and Clayton, Richard},
  booktitle={Peer-to-Peer Computing, 2006. {P2P} 2006. Sixth {IEEE} International Conference on},
  pages={69--72},
  year={2006},
  organization={IEEE}
}

@conference {Dingledine:2006:usability,
	title = {Anonymity Loves Company: Usability and the Network Effect},
	booktitle = {Proceedings of the Fifth Workshop on the Economics of Information Security ({WEIS} 2006)},
	year = {2006},
	month = {June},
	address = {Cambridge, UK},
	author = {Roger Dingledine and Nick Mathewson},
	editor = {Ross Anderson}
}

@Inbook{Dwork:2006:DiffPrivacy,
author={Dwork, Cynthia},
editor={Bugliesi, Michele
and Preneel, Bart
and Sassone, Vladimiro
and Wegener, Ingo},
title={Differential Privacy},
bookTitle={Automata, Languages and Programming: 33rd International Colloquium, ICALP 2006, Venice, Italy, July 10-14, 2006, Proceedings, Part II},
year={2006},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={1--12},
isbn={978-3-540-35908-1},
doi={10.1007/11787006_1},
url={http://dx.doi.org/10.1007/11787006_1}
}

@incollection{Goldberg:2006:Tor-Auth,
year={2006},
booktitle={Privacy Enhancing Technologies},
volume={4258},
series={Lecture Notes in Computer Science},
editor={Danezis, George and Golle, Philippe},
title={On the Security of the {Tor} Authentication Protocol},
publisher={Springer Berlin Heidelberg},
author={Goldberg, Ian},
pages={316-331},
}

@inproceedings{Liberatore:2006:TA,
 author = {Liberatore, Marc and Levine, Brian Neil},
 title = {Inferring the Source of Encrypted {HTTP} Connections},
 booktitle = {Proceedings of the 13th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '06},
 year = {2006},
 location = {Alexandria, Virginia, USA},
 pages = {255--263},
 numpages = {9},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Nambiar:2006:Salsa,
 author = {Nambiar, Arjun and Wright, Matthew},
 title = {Salsa: A Structured Approach to Large-scale Anonymity},
 booktitle = {Proceedings of the 13th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '06},
 year = {2006},
 location = {Alexandria, Virginia, USA},
 pages = {17--26},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Overlier:2006:Tor-hs,
  title = {Locating Hidden Servers}, 
  author = {Lasse {\O}verlier and Paul Syverson}, 
  booktitle = {Proceedings of the 2006 {IEEE} Symposium on Security and Privacy ({SP})}, 
  year = {2006}, 
  month = {May}, 
  publisher = {IEEE}
}

@ARTICLE{Sampigethaya:2006:MixNet, 
author={Sampigethaya, K. and Poovendran, R.}, 
journal={Proceedings of the IEEE}, 
title={A Survey on Mix Networks and Their Secure Applications}, 
year={2006}, 
month={December}, 
volume={94}, 
number={12}, 
pages={2142-2181}, 
}

@inproceedings{Shmatikov:2006:MinEntropy,
 author = {Shmatikov, Vitaly and Wang, Ming-Hsiu},
 title = {Measuring Relationship Anonymity in Mix Networks},
 booktitle = {Proceedings of the 5th ACM Workshop on Privacy in Electronic Society},
 series = {WPES '06},
 year = {2006},
 isbn = {1-59593-556-8},
 location = {Alexandria, Virginia, USA},
 pages = {59--62},
 numpages = {4},
 url = {http://doi.acm.org/10.1145/1179601.1179611},
 doi = {10.1145/1179601.1179611},
 acmid = {1179611},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymity, mix networks, privacy},
} 

@incollection{Shmatikov:2006:Mix-Attacks,
year={2006},
booktitle={Computer Security – {ESORICS} 2006},
volume={4189},
series={Lecture Notes in Computer Science},
editor={Gollmann, Dieter and Meier, Jan and Sabelfeld, Andrei},
title={Timing Analysis in Low-Latency Mix Networks: Attacks and Defenses},
publisher={Springer Berlin Heidelberg},
author={Shmatikov, Vitaly and Wang, Ming-Hsiu},
pages={18-33},
}

@incollection{Tabriz:2006:Breaking-MorphMix,
year={2006},
booktitle={Privacy Enhancing Technologies},
volume={4258},
series={Lecture Notes in Computer Science},
editor={Danezis, George and Golle, Philippe},
title={Breaking the Collusion Detection Mechanism of {MorphMix}},
publisher={Springer Berlin Heidelberg},
author={Tabriz, Parisa and Borisov, Nikita},
pages={368-383},
}

@techreport{Wang:2006:Myrmic,
  title={Myrmic: Provably secure and efficient {DHT} routing},
  author={Peng Wang and Ivan Osipkov and Nicholas Hopper and Yongdae Kim},
  year={2006},
  institution={DTC},
}

@article{Yu:2006:Sybil,
 author = {Yu, Haifeng and Kaminsky, Michael and Gibbons, Phillip B. and Flaxman, Abraham},
 title = {{SybilGuard}: Defending Against Sybil Attacks via Social Networks},
 journal = {SIGCOMM Comput. Commun. Rev.},
 month = {October},
 volume = {36},
 number = {4},
 month = {August},
 year = {2006},
 pages = {267--278},
 numpages = {12},
 publisher = {ACM},
}

@incollection{Boehme:2005:MIXvsP2P,
year={2005},
booktitle={Privacy Enhancing Technologies},
volume={3424},
series={Lecture Notes in Computer Science},
editor={Martin, David and Serjantov, Andrei},
title={On the {PET} Workshop Panel “Mix Cascades Versus Peer-to-Peer: Is One Concept Superior?”},
publisher={Springer Berlin Heidelberg},
author={B{\"{o}}hme, Rainer and Danezis, George and D{\'{\i}}az, Claudia and K{\"{o}}psell, Stefan and Pfitzmann, Andreas},
pages={243-255},
}

@inproceedings{Borisov:2005:APM,
 author = {Borisov, Nikita},
 title = {An Analysis of Parallel Mixing with Attacker-controlled Inputs},
 booktitle = {Proceedings of the 5th International Conference on Privacy Enhancing Technologies},
 series = {PET'05},
 year = {2006},
 isbn = {3-540-34745-3, 978-3-540-34745-3},
 location = {Cavtat, Croatia},
 pages = {12--25},
 numpages = {14},
 url = {http://dx.doi.org/10.1007/11767831_2},
 doi = {10.1007/11767831_2},
 acmid = {2180085},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 



@incollection{Camenisch:2005:Formal-Onion,
year={2005},
booktitle={Advances in Cryptology - {CRYPTO} 2005},
volume={3621},
series={Lecture Notes in Computer Science},
editor={Shoup, Victor},
title={A Formal Treatment of Onion Routing},
publisher={Springer Berlin Heidelberg},
author={Camenisch, Jan and Lysyanskaya, Anna},
pages={169-187},
}

@incollection{Danezis:2005:Attacks,
year={2005},
booktitle={Information Hiding},
volume={3200},
series={Lecture Notes in Computer Science},
editor={Fridrich, Jessica},
title={Statistical Disclosure or Intersection Attacks on Anonymity Systems},
publisher={Springer Berlin Heidelberg},
author={Danezis, George and Serjantov, Andrei},
pages={293-308},
}

@incollection{Danezis:2005:Time-Mix,
year={2005},
booktitle={Privacy Enhancing Technologies},
volume={3424},
series={Lecture Notes in Computer Science},
editor={Martin, David and Serjantov, Andrei},
title={The Traffic Analysis of Continuous-Time Mixes},
publisher={Springer Berlin Heidelberg},
author={Danezis, George},
pages={35-50},
}

@incollection{Diaz:2005:DummyTraffic,
year={2005},
booktitle={Information Hiding},
volume={3200},
series={Lecture Notes in Computer Science},
editor={Fridrich, Jessica},
title={Reasoning About the Anonymity Provided by Pool Mixes That Generate Dummy Traffic},
publisher={Springer Berlin Heidelberg},
author={D{\'{\i}}az, Claudia and Preneel, Bart},
pages={309-325},
}

@incollection{Dingledine:2005:SyncBatchingCascadeFRoute,
year={2005},
isbn={978-3-540-26203-9},
booktitle={Privacy Enhancing Technologies},
volume={3424},
series={Lecture Notes in Computer Science},
editor={Martin, David and Serjantov, Andrei},
doi={10.1007/11423409_12},
title={Synchronous Batching: From Cascades to Free Routes},
url={http://dx.doi.org/10.1007/11423409_12},
publisher={Springer Berlin Heidelberg},
author={Dingledine, Roger and Shmatikov, Vitaly and Syverson, Paul},
pages={186-206},
language={English}
}

@Inbook{Klonowski:2005:ProvableMixnets,
author={Klonowski, Marek and Kuty{\l}owski, Miros{\l}aw},
editor={Barni, Mauro and Herrera-Joancomart{\'i}, Jordi and Katzenbeisser, Stefan and P{\'e}rez-Gonz{\'a}lez, Fernando},
title={Provable Anonymity for Networks of Mixes},
bookTitle={Information Hiding: 7th International Workshop, IH 2005, Barcelona, Spain, June 6-8, 2005. Revised Selected Papers},
year={2005},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={26--38},
isbn={978-3-540-31481-3},
doi={10.1007/11558859_3},
url={http://dx.doi.org/10.1007/11558859_3}
}



@incollection{Mathewson:2005:Traffic-Analysis,
year={2005},
booktitle={Privacy Enhancing Technologies},
volume={3424},
series={Lecture Notes in Computer Science},
editor={Martin, David and Serjantov, Andrei},
title={Practical Traffic Analysis: Extending and Resisting Statistical Disclosure},
publisher={Springer Berlin Heidelberg},
author={Mathewson, Nick and Dingledine, Roger},
pages={17-34},
}

@INPROCEEDINGS{Murdoch:2005:Traffic-Analysis,
author={Murdoch, S.J. and Danezis, G.}, 
booktitle={Security and Privacy, 2005 {IEEE} Symposium on}, 
title={Low-cost traffic analysis of {Tor}}, 
year={2005}, 
month={May}, 
pages={183-195}, 
}

@inproceedings{OConnor:2005,
  author    = {Luke O'Connor},
  title     = {On Blending Attacks for Mixes with Memory},
  booktitle = {Information Hiding, 7th International Workshop, {IH} 2005, Barcelona, Spain, June 6-8, 2005, Revised Selected Papers},
  year      = {2005},
  pages     = {39--52}
}

@incollection{Zhu:2005:Mix-Correlation,
year={2005},
booktitle={Privacy Enhancing Technologies},
volume={3424},
series={Lecture Notes in Computer Science},
editor={Martin, David and Serjantov, Andrei},
title={On Flow Correlation Attacks and Countermeasures in Mix Networks},
publisher={Springer Berlin Heidelberg},
author={Zhu, Ye and Fu, Xinwen and Graham, Bryan and Bettati, Riccardo and Zhao, Wei},
pages={207-225},
}

@inproceedings{Danezis:2004:Serjantov,
  author    = {George Danezis and
               Andrei Serjantov},
  title     = {Statistical Disclosure or Intersection Attacks on Anonymity Systems},
  booktitle = {Information Hiding, 6th International Workshop, {IH} 2004, Toronto, Canada, May 23-25, 2004, Revised Selected Papers},
  year      = {2004},
  pages     = {293--308}
}

@techreport{Danezis:2004:designing,
  title={Designing and attacking anonymous communication systems},
  author={Danezis, George},
  institution={University of Cambridge, Computer Laboratory},
  year={2004}
}

@inproceedings{Diaz:2004,
  author    = {Claudia D{\'{\i}}az and
               Bart Preneel},
  title     = {Taxonomy of Mixes and Dummy Traffic},
  booktitle = {Information Security Management, Education and Privacy, {IFIP} 18th World Computer Congress, {TC11} 19th International Information Security Workshops, 22-27 August 2004, Toulouse, France},
  year      = {2004},
  pages     = {215--230}
}

@incollection{Diaz:2004:Two-Mix,
year={2004},
booktitle={Computer Security - {ESORICS} 2004},
volume={3193},
series={Lecture Notes in Computer Science},
editor={Samarati, Pierangela and Ryan, Peter and Gollmann, Dieter and Molva, Refik},
title={Comparison Between Two Practical Mix Designs},
publisher={Springer Berlin Heidelberg},
author={D{\'{\i}}az, Claudia and Sassaman, Len and Dewitte, Evelyne},
pages={141-159},
}

@inproceedings{Dingledine:2004,
  author    = {Roger Dingledine and
               Vitaly Shmatikov and
               Paul F. Syverson},
  title     = {Synchronous Batching: From Cascades to Free Routes},
  booktitle = {Privacy Enhancing Technologies, 4th International Workshop, {PET} 2004, Toronto, Canada, May 26-28, 2004, Revised Selected Papers},
  year      = {2004},
  pages     = {186--206}
}

@inproceedings{Dingledine:2004:Tor,
 author = {Dingledine, Roger and Mathewson, Nick and Syverson, Paul},
 title = {Tor: The Second-generation Onion Router},
 booktitle = {Proceedings of the 13th Conference on {USENIX} Security Symposium - Volume 13},
 series = {{SSYM} '04},
 year = {2004},
pages = {303--320},
 publisher = {USENIX Association},
}

@inproceedings{Feamster:2004:LocationDiversity,
 author = {Feamster, Nick and Dingledine, Roger},
 title = {Location Diversity in Anonymity Networks},
 booktitle = {Proceedings of the 2004 {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '04},
 year = {2004},
 location = {Washington DC, USA},
 pages = {66--76},
 numpages = {11},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Levine:2004:timingattacks,
  author    = {Brian Neil Levine and
               Michael K. Reiter and
               Chenxi Wang and
               Matthew K. Wright},
  title     = {Timing Attacks in Low-Latency Mix Systems (Extended Abstract)},
  booktitle = {Financial Cryptography, 8th International Conference, {FC} 2004, Key
               West, FL, USA, February 9-12, 2004. Revised Papers},
  pages     = {251--265},
  year      = {2004}
}

@incollection{Golle:2005:ReputeableMixes,
author={Golle, Philippe},
editor={Martin, David and Serjantov, Andrei},
chapter={Reputable Mix Networks},
title={Privacy Enhancing Technologies: 4th International Workshop, PET 2004, Toronto, Canada, May 26-28, 2004. Revised Selected Papers},
year={2005},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={51--62},
isbn={978-3-540-31960-3},
doi={10.1007/11423409_4},
url={http://dx.doi.org/10.1007/11423409_4}
}


@incollection{Golle:2004:DC,
year={2004},
booktitle={Advances in Cryptology - {EUROCRYPT} '04},
volume={3027},
series={Lecture Notes in Computer Science},
editor={Cachin, Christian and Camenisch, JanL.},
title={Dining Cryptographers Revisited},
publisher={Springer Berlin Heidelberg},
author={Golle, Philippe and Juels, Ari},
pages={456-473},
}

@incollection{Golle:2004:Mix,
year={2004},
booktitle={Topics in Cryptology - {CT-RSA} 2004},
volume={2964},
series={Lecture Notes in Computer Science},
editor={Okamoto, Tatsuaki},
title={Universal Re-encryption for {Mixnets}},
publisher={Springer Berlin Heidelberg},
author={Golle, Philippe and Jakobsson, Markus and Juels, Ari and Syverson, Paul},
pages={163-178},
}

@inproceedings{Golle:2004:ParallelMixes,
 author = {Golle, Philippe and Juels, Ari},
 title = {Parallel Mixing},
 booktitle = {Proceedings of the 11th ACM Conference on Computer and Communications Security},
 series = {CCS '04},
 year = {2004},
 isbn = {1-58113-961-6},
 location = {Washington DC, USA},
 pages = {220--226},
 numpages = {7},
 url = {http://doi.acm.org/10.1145/1030083.1030113},
 doi = {10.1145/1030083.1030113},
 acmid = {1030113},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymity, mixnet, parallel execution, permutation, privacy},
} 



@phdthesis{Groth:2004:ZK,
  title={Honest verifier zero-knowledge arguments applied},
  author={Groth, Jens},
  year={2004},
  school={University of Aarhus, Denmark},
}

@incollection{Levine:2004:Mix-Attack,
year={2004},
booktitle={Financial Cryptography},
volume={3110},
series={Lecture Notes in Computer Science},
editor={Juels, Ari},
title={Timing Attacks in Low-Latency Mix Systems},
publisher={Springer Berlin Heidelberg},
author={Levine, BrianN. and Reiter, MichaelK. and Wang, Chenxi and Wright, Matthew},
pages={251-265},
}

@inproceedings{Mislove:2004:AP3,
	author    = {Alan Mislove and
	Gaurav Oberoi and
	Ansley Post and
	Charles Reis and
	Peter Druschel and
	Dan S. Wallach},
	title     = {{AP3:} cooperative, decentralized anonymous communication},
	booktitle = {Proceedings of the 11st {ACM} {SIGOPS} European Workshop, Leuven,
	Belgium, September 19-22, 2004},
	pages     = {30},
	year      = {2004}
}

@incollection{Rennhard:2004:MorphMix,
year={2004},
booktitle={Financial Cryptography},
volume={3110},
series={Lecture Notes in Computer Science},
editor={Juels, Ari},
title={Practical Anonymity for the Masses with MorphMix},
publisher={Springer Berlin Heidelberg},
author={Rennhard, Marc and Plattner, Bernhard},
pages={233-250},
}

@techreport{Serjantov:2004:Anonymity,
  title={On the anonymity of anonymity systems},
  author={Serjantov, Andrei},
  institution={University of Cambridge, Computer Laboratory},
  year={2004},
  month={October},
}

@article{Shmatikov:2004:Analysis,
  author    = {Vitaly Shmatikov},
  title     = {Probabilistic analysis of an anonymity system},
  journal   = {Journal of Computer Security},
  volume    = {12},
  number    = {3-4},
  pages     = {355--377},
  year      = {2004},
}

@inproceedings{Singh:2004:EclipseAttacks,
 author = {Singh, Atul and Castro, Miguel and Druschel, Peter and Rowstron, Antony},
 title = {Defending Against Eclipse Attacks on Overlay Networks},
 booktitle = {Proceedings of the 11th Workshop on {ACM SIGOPS European} Workshop},
 series = {{EW} '11},
 year = {2004},
 location = {Leuven, Belgium},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@incollection{Wang:2004:Signature,
year={2004},
booktitle={Information Security and Privacy},
volume={3108},
series={Lecture Notes in Computer Science},
editor={Wang, Huaxiong and Pieprzyk, Josef and Varadharajan, Vijay},
title={Linkable Spontaneous Anonymous Group Signature for Ad Hoc Groups},
publisher={Springer Berlin Heidelberg},
author={Liu, JosephK. and Wei, VictorK. and Wong, DuncanS.},
pages={325-335},
}

@incollection{Wikstroem:2004:Five-Mix-Attacks,
year={2004},
booktitle={Selected Areas in Cryptography},
volume={3006},
series={Lecture Notes in Computer Science},
editor={Matsui, Mitsuru and Zuccherato, RobertJ.},
title={Five Practical Attacks for “Optimistic Mixing for Exit-Polls”},
publisher={Springer Berlin Heidelberg},
author={Wikstr{\"o}m, Douglas},
pages={160-174},
}

@article{Wright:2004:PredecessorAttack,
 author = {Wright, Matthew K. and Adler, Micah and Levine, Brian Neil and Shields, Clay},
 title = {The Predecessor Attack: An Analysis of a Threat to Anonymous Communications Systems},
 journal = {ACM Trans. Inf. Syst. Secur.},
 volume = {7},
 number = {4},
 month = {Novmeber},
 year = {2004},
 pages = {489--522},
 numpages = {34},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@incollection{Acquisti:2003:Economics,
year={2003},
booktitle={Financial Cryptography},
volume={2742},
series={Lecture Notes in Computer Science},
editor={Wright, RebeccaN.},
title={On the Economics of Anonymity},
publisher={Springer Berlin Heidelberg},
author={Acquisti, Alessandro and Dingledine, Roger and Syverson, Paul},
pages={84-102},
}

@MISC{Bennett:2003:ECRS,
    author = {Krista Bennett and Christian Grothoff and Tzvetan Horozov and J. T. Lindgren},
    title = {An Encoding for Censorship-Resistant Sharing},
    year = {2003}
}

@incollection{Bennett:2003:GAP,
year={2003},
booktitle={Privacy Enhancing Technologies},
volume={2760},
series={Lecture Notes in Computer Science},
editor={Dingledine, Roger},
title={gap – Practical Anonymous Networking},
publisher={Springer Berlin Heidelberg},
author={Bennett, Krista and Grothoff, Christian},
pages={141-160},
}

@incollection{Berthold:2003:Intersection-Attack,
year={2003},
booktitle={Privacy Enhancing Technologies},
volume={2482},
series={Lecture Notes in Computer Science},
editor={Dingledine, Roger and Syverson, Paul},
title={Dummy Traffic against Long Term Intersection Attacks},
publisher={Springer Berlin Heidelberg},
author={Berthold, Oliver and Langos, Heinrich},
pages={110-128},
}

@inproceedings{Danezis:2003,
  author    = {George Danezis},
  title     = {Mix-Networks with Restricted Routes},
  booktitle = {Privacy Enhancing Technologies, Third International Workshop, {PET} 2003, Dresden, Germany, March 26-28, 2003, Revised Papers},
  year      = {2003},
  pages     = {1--17},
}

@inproceedings{Danezis:2003:disclosure,
  author    = {George Danezis},
  title     = {Statistical Disclosure Attacks},
  booktitle = {Security and Privacy in the Age of Uncertainty, {IFIP} {TC11} 18\({}^{\mbox{th}}\) International Conference on Information Security ({SEC} '03), May 26-28, 2003, Athens, Greece},
  year      = {2003},
  pages     = {421--426}
}

@inproceedings{Danezis:2003:Heartbeat,
 author = {Danezis, George and Sassaman, Len},
 title = {Heartbeat Traffic to Counter (N-1) Attacks: Red-green-black Mixes},
 booktitle = {Proceedings of the 2003 {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '03},
 year = {2003},
 location = {Washington, DC},
 pages = {89--93},
 numpages = {5},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Danezis:2003:mixminion,
  author    = {George Danezis and
               Roger Dingledine and
               Nick Mathewson},
  title     = {Mixminion: Design of a Type {III} Anonymous Remailer Protocol},
  booktitle = {2003 {IEEE} Symposium on Security and Privacy ({SP} 2003), 11-14 May 2003, Berkeley, CA, {USA}},
  year      = {2003},
  pages     = {2--15},
}

@incollection{Diaz:2003:Generalising-Mixes,
year={2003},
booktitle={Privacy Enhancing Technologies},
volume={2760},
series={Lecture Notes in Computer Science},
editor={Dingledine, Roger},
title={Generalising Mixes},
publisher={Springer Berlin Heidelberg},
author={D{\'{\i}}az, Claudia and Serjantov, Andrei},
pages={18-31},
}

@incollection{Diaz:2003:Measurement,
year={2003},
booktitle={Privacy Enhancing Technologies},
volume={2482},
series={Lecture Notes in Computer Science},
editor={Dingledine, Roger and Syverson, Paul},
title={Towards Measuring Anonymity},
publisher={Springer Berlin Heidelberg},
author={D{\'{\i}}az, Claudia and Seys, Stefaan and Claessens, Joris and Preneel, Bart},
pages={54-68},
}

@inproceedings{Diaz:2003:Serjantov,
  author    = {Claudia D{\'{\i}}az and
               Andrei Serjantov},
  title     = {Generalising Mixes},
  booktitle = {Privacy Enhancing Technologies, Third International Workshop, {PET} 2003, Dresden, Germany, March 26-28, 2003, Revised Papers},
  year      = {2003},
  pages     = {18--31}
}



@techreport{Goel:2003:Herbivore,
  title={Herbivore: A scalable and efficient protocol for anonymous communication},
  author={Goel, Sharad and Robson, Mark and Polte, Milo and Sirer, Emin},
  year={2003},
  institution={Cornell University}
}

@article {Grothoff:2003:EconomicModelGnuNet,
	title = {An Excess-Based Economic Model for Resource Allocation in Peer-to-Peer Networks},
	journal = {Wirtschaftsinformatik},
	volume = {3-2003},
	year = {2003},
	month = {June},
	publisher = {Vieweg-Verlag},
	abstract = {This paper describes economic aspects of GNUnet, a peer-to-peer framework for anonymous distributed file-sharing.  GNUnet is decentralized; all nodes are equal peers. In particular, there are no trusted entities in the network. This paper describes an economic model to perform resource allocation and defend against malicious
participants in this context.  The approach presented does not use credentials or payments; rather, it is based on trust.  The design is much like that of a cooperative game in which peers take the role of players. Nodes must cooperate to achieve individual goals.  In such a scenario, it is important to be able to distinguish between nodes exhibiting friendly behavior and those exhibiting malicious behavior.

GNUnet aims to provide anonymity for its users.  Its design
makes it hard to link a transaction to the node where it originated from.  While anonymity requirements make a global view of the end-points of a transaction infeasible, the local link-to-link messages can be fully authenticated.  Our economic model is based entirely on this local view of the network and takes only local
decisions.
},
	keywords = {anonymity, file-sharing, GNUnet},
	url = {http://grothoff.org/christian/ebe.pdf},
	author = {Christian Grothoff}
}

@misc{moller:2003:mixmaster,
  title={Mixmaster protocol - version 2},
  author={M{\"o}ller, Ulf and Cottrell, Lance and Palfrader, Peter and Sassaman, Len},
  year={2003}
}

@incollection{Serjantov:2003:Attacks,
year={2003},
booktitle={Information Hiding},
volume={2578},
series={Lecture Notes in Computer Science},
editor={Petitcolas, FabienA.P.},
title={From a Trickle to a Flood: Active Attacks on Several Mix Types},
publisher={Springer Berlin Heidelberg},
author={Serjantov, Andrei and Dingledine, Roger and Syverson, Paul},
pages={36-52},
}

@incollection{Serjantov:2003:PassiveAttack,
year={2003},
booktitle={Computer Security – {ESORICS} 2003},
volume={2808},
series={Lecture Notes in Computer Science},
editor={Snekkenes, Einar and Gollmann, Dieter},
title={Passive Attack Analysis for Connection-Based Anonymity Systems},
publisher={Springer Berlin Heidelberg},
author={Serjantov, Andrei and Sewell, Peter},
pages={116-131},
}

@incollection{Serjantov:2003:Metric,
year={2003},
booktitle={Privacy Enhancing Technologies},
volume={2482},
series={Lecture Notes in Computer Science},
editor={Dingledine, Roger and Syverson, Paul},
title={Towards an Information Theoretic Metric for Anonymity},
publisher={Springer Berlin Heidelberg},
author={Serjantov, Andrei and Danezis, George},
pages={41-53},
}
	
@inproceedings{Serjantov:2003:Newman,
  author    = {Andrei Serjantov and
               Richard E. Newman},
  title     = {On the Anonymity of Timed Pool Mixes},
  booktitle = {Security and Privacy in the Age of Uncertainty, {IFIP} {TC11} 18\({}^{\mbox{th}}\) International Conference on Information Security ({SEC} 2003), May 26-28, 2003, Athens, Greece},
  year      = {2003},
  pages     = {427--434}
}

@inproceedings{Wang:2003:Correlation-Traffic,
 author = {Wang, Xinyuan and Reeves, Douglas S.},
 title = {Robust Correlation of Encrypted Attack Traffic Through Stepping Stones by Manipulation of Interpacket Delays},
 booktitle = {Proceedings of the 10th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '03},
 year = {2003},
 location = {Washington D.C., USA},
 pages = {20--29},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@INPROCEEDINGS{Wright:2003:defending-predecessor-attacks, 
author={Wright, M. and Adler, M. and Levine, B.N. and Shields, C.}, 
booktitle={Security and Privacy ({SP}), 2003. Proceedings. 2003 Symposium on}, 
title={Defending anonymous communications against passive logging attacks}, 
year={2003}, 
month={May}, 
pages={28-41},
}

@article {Bennett:2002:GN,
	title = {The GNet Whitepaper},
	year = {2002},
	month = {June},
	institution = {Purdue University},
	type = {Technical report},
	author = {Krista Bennett and Tiberius Stef and Christian Grothoff and Tzvetan Horozov and Ioana Patrascu}
}

@inproceedings{Boneh:2002:AEC,
 author = {Boneh, Dan and Golle, Philippe},
 title = {Almost Entirely Correct Mixing with Applications to Voting},
 booktitle = {Proceedings of the 9th ACM Conference on Computer and Communications Security},
 series = {CCS '02},
 year = {2002},
 isbn = {1-58113-612-9},
 location = {Washington, DC, USA},
 pages = {68--77},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/586110.586121},
 doi = {10.1145/586110.586121},
 acmid = {586121},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {electronic voting, mix networks},
} 


@article{Castro:2002:Eclipse,
 author = {Castro, Miguel and Druschel, Peter and Ganesh, Ayalvadi and Rowstron, Antony and Wallach, Dan S.},
 title = {Secure Routing for Structured Peer-to-peer Overlay Networks},
 journal = {SIGOPS Oper. Syst. Rev.},
 issue_date = {Winter 2002},
 volume = {36},
 number = {SI},
 month = dec,
 year = {2002},
 issn = {0163-5980},
 pages = {299--314},
 numpages = {16},
 url = {http://doi.acm.org/10.1145/844128.844156},
 doi = {10.1145/844128.844156},
 acmid = {844156},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@inproceedings{Danezis:2002:FSec-Mix,
  title={Forward secure mixes},
  author={Danezis, George},
  booktitle={Nordic workshop on Secure IT Systems (Norsec 2002},
  year={2002},
}

@inproceedings{Diaz:2002:EntropyMetric,
 author = {D\'{\i}az, Claudia and Seys, Stefaan and Claessens, Joris and Preneel, Bart},
 title = {Towards Measuring Anonymity},
 booktitle = {Proceedings of the 2Nd International Conference on Privacy Enhancing Technologies},
 series = {PET'02},
 year = {2003},
 isbn = {3-540-00565-X},
 location = {San Francisco, CA, USA},
 pages = {54--68},
 numpages = {15},
 url = {http://dl.acm.org/citation.cfm?id=1765299.1765304},
 acmid = {1765304},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 


@incollection{Dingledine:2003:Reliable-Mix,
year={2002},
booktitle={Financial Cryptography},
volume={2357},
series={Lecture Notes in Computer Science},
editor={Blaze, Matt},
title={Reliable {MIX} Cascade Networks through Reputation},
publisher={Springer Berlin Heidelberg},
author={Dingledine, Roger and Syverson, Paul},
pages={253-268},
}

@incollection{Douceur:2002:Sybil,
year={2002},
booktitle={Peer-to-Peer Systems},
volume={2429},
series={Lecture Notes in Computer Science},
editor={Druschel, Peter and Kaashoek, Frans and Rowstron, Antony},
title={The Sybil Attack},
publisher={Springer Berlin Heidelberg},
author={Douceur, JohnR.},
pages={251-260},
}

@inproceedings{Freedman:2002:Tarzan,
 author = {Freedman, Michael J. and Morris, Robert},
 title = {Tarzan: A Peer-to-peer Anonymizing Network Layer},
 booktitle = {Proceedings of the 9th {ACM} Conference on Computer and Communications Security},
 series = {CCS '02},
 year = {2002},
 pages = {193--206},
 numpages = {14},
 publisher = {ACM},
}

@inproceedings{IPTPS:2002:Tarzan,
  author    = {Michael J. Freedman and
               Emil Sit and
               Josh Cates and
               Robert Morris},
  title     = {Introducing Tarzan, a Peer-to-Peer Anonymizing Network Layer},
  booktitle = {Peer-to-Peer Systems, First International Workshop, {IPTPS} 2002,
               Cambridge, MA, USA, March 7-8, 2002, Revised Papers},
  pages     = {121--129},
  year      = {2002}
}

@incollection{Golle:2002:Mix,
year={2002},
booktitle={Advances in Cryptology - {ASIACRYPT} 2002},
volume={2501},
series={Lecture Notes in Computer Science},
editor={Zheng, Yuliang},
title={Optimistic Mixing for Exit-Polls},
publisher={Springer Berlin Heidelberg},
author={Golle, Philippe and Zhong, Sheng and Boneh, Dan and Jakobsson, Markus and Juels, Ari},
pages={451-465},
}

@inproceedings{Jakobsson:2002:Voting,
  author    = {Markus Jakobsson and
               Ari Juels and
               Ronald L. Rivest},
  title     = {Making Mix Nets Robust for Electronic Voting by Randomized Partial
               Checking},
  booktitle = {Proceedings of the 11th {USENIX} Security Symposium, San Francisco,
               CA, USA, August 5-9, 2002},
  pages     = {339--353},
  year      = {2002}
}

@inproceedings{Kesdogan:2002:limits,
  author    = {Dogan Kesdogan and
               Dakshi Agrawal and
               Stefan Penz},
  title     = {Limits of Anonymity in Open Environments},
  booktitle = {Information Hiding, 5th International Workshop, {IH} 2002, Noordwijkerhout,
               The Netherlands, October 7-9, 2002, Revised Papers},
  pages     = {53--69},
  year      = {2002}
}

@article{Levine:2002:Hordes,
  author    = {Brian Neil Levine and
               Clay Shields},
  title     = {Hordes: a Multicast-Based Protocol for Anonymity},
  journal   = {Journal of Computer Security},
  volume    = {10},
  number    = {3},
  pages     = {213--240},
  year      = {2002},
}

@inproceedings{Maymounkov:2002:Kademlia,
 author = {Maymounkov, Petar and Mazi\`{e}res, David},
 title = {Kademlia: A Peer-to-Peer Information System Based on the XOR Metric},
 booktitle = {Revised Papers from the First International Workshop on Peer-to-Peer Systems},
 series = {{IPTPS} '01},
 year = {2002},
 pages = {53--65},
 numpages = {13},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@Inbook{Czumaj:2001:SwitchingNetowrksRandomPermutations,
author={Czumaj, Artur and Kanarek, Przemka and Lory{\'{s}}, Krzysztof and Kutylowski, Miroslaw},
editor={Du, Ding Zhu and Ngo, Hung Q.},
title={Switching Networks for Generating Random Permutations},
bookTitle={Switching Networks: Recent Advances},
year={2001},
publisher={Springer US},
address={Boston, MA},
pages={25--61},
isbn={978-1-4613-0281-0},
doi={10.1007/978-1-4613-0281-0_2},
url={http://dx.doi.org/10.1007/978-1-4613-0281-0_2}
}


@inproceedings{Rennhard:2002:MorphMix,
 author = {Rennhard, Marc and Plattner, Bernhard},
 title = {Introducing {MorphMix}: Peer-to-peer Based Anonymous Internet Usage with Collusion Detection},
 booktitle = {Proceedings of the 2002 {ACM} Workshop on Privacy in the Electronic Society},
 series = {{WPES} '02},
 year = {2002},
 location = {Washington, DC},
 pages = {91--102},
 numpages = {12},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Serjantov:2002,
  author    = {Andrei Serjantov and
               Roger Dingledine and
               Paul F. Syverson},
  title     = {From a Trickle to a Flood: Active Attacks on Several Mix Types},
  booktitle = {Information Hiding, 5th International Workshop, {IH} 2002, Noordwijkerhout,
               The Netherlands, October 7-9, 2002, Revised Papers},
  year      = {2002},
  pages     = {36--52}
}

@INPROCEEDINGS{Sherwood:2002:P5, 
author={Sherwood, R. and Bhattacharjee, B. and Srinivasan, A.}, 
booktitle={Security and Privacy, 2002. Proceedings. 2002 IEEE Symposium on}, 
title={P5: A protocol for scalable anonymous communication}, 
year={2002}, 
pages={58-70}, 
}

@inproceedings{Shmatikov:2002:probabilisticanalysis,
author = {Vitaly Shmatikov},
title = {Probabilistic Analysis of Anonymity},
booktitle = {In Proc. 15th Computer Security Foundations Workshop},
year = {2002},
pages = {119--128},
publisher = {Society Press}
}

@INPROCEEDINGS{Sun:2002:web-stat,
author={Sun, Q. and Simon, D.R. and Yi-Min Wang and Russell, W. and Padmanabhan, V.N. and Lili Qiu}, 
booktitle={Security and Privacy ({SP}), 2002. Proceedings. 2002 {IEEE} Symposium on}, 
title={Statistical identification of encrypted Web browsing traffic}, 
year={2002}, 
pages={19-30},
}

@incollection{Wang:2002:Correlation,
year={2002},
booktitle={Computer Security - {ESORICS} 2002},
volume={2502},
series={Lecture Notes in Computer Science},
editor={Gollmann, Dieter and Karjoth, G{\"{u}}nter and Waidner, Michael},
title={Inter-Packet Delay Based Correlation for Tracing Encrypted Connections through Stepping Stones},
publisher={Springer Berlin Heidelberg},
author={Wang, Xinyuan and Reeves, DouglasS. and Wu, S.Felix},
pages={244-263},
}

@inproceedings{Wright:2002:Degradation,
  author    = {Matthew Wright and
               Micah Adler and
               Brian Neil Levine and
               Clay Shields},
  title     = {An Analysis of the Degradation of Anonymous Protocols},
  booktitle = {Proceedings of the Network and Distributed System Security Symposium,
               {NDSS} 2002, San Diego, California, {USA}},
  year      = {2002},
  crossref  = {DBLP:conf/ndss/2002},
}
@proceedings{DBLP:conf/ndss/2002,
  title     = {Proceedings of the Network and Distributed System Security Symposium,
               {NDSS} 2002, San Diego, California, {USA}},
  publisher = {The Internet Society},
  year      = {2002},
}

@INPROCEEDINGS{Zou:2002:routingclassification,
    author = {Xukai Zou and Byrav Ramamurthy and Spyros Magliveras},
    title = {Routing techniques in wireless ad hoc networks - classification and comparison},
    booktitle = {Proceedings of the Sixth World Multiconference on Systemics, Cybernetics, and Informatics ({SCI} 2002},
    year = {2002}
}

@misc{Back:2001:Freedom21,
  title={Freedom 2.1 security issues and analysis},
  author={Back, Adam and Goldberg, Ian and Shostack, Adam},
  note={White Paper},
  year={2001}
}

@incollection{Back:2001:Tradeoff,
year={2001},
booktitle={Information Hiding},
volume={2137},
series={Lecture Notes in Computer Science},
editor={Moskowitz, IraS.},
title={Traffic Analysis Attacks and Trade-Offs in Anonymity Providing Systems},
publisher={Springer Berlin Heidelberg},
author={Back, Adam and  M{\"{o}}ller, Ulf and Stiglic, Anton},
pages={245-257},
}

@incollection{Berthold:2001:Web-Mixes,
year={2001},
booktitle={Designing Privacy Enhancing Technologies},
volume={2009},
series={Lecture Notes in Computer Science},
editor={Federrath, Hannes},
title={{Web MIXes}: A System for Anonymous and Unobservable Internet Access},
publisher={Springer Berlin Heidelberg},
author={Berthold, Oliver and Federrath, Hannes and K{\"{o}}psell, Stefan},
pages={115-129},
}

@incollection{Berthold:2001:Disadvantages,
year={2001},
booktitle={Designing Privacy Enhancing Technologies},
volume={2009},
series={Lecture Notes in Computer Science},
editor={Federrath, Hannes},
title={The Disadvantages of Free {MIX} Routes and How to Overcome Them},
publisher={Springer Berlin Heidelberg},
author={Berthold, Oliver and Pfitzmann, Andreas and Standtke, Ronny},
pages={30-45},
}

@incollection{Boneh:2001:IBE,
year={2001},
booktitle={Advances in Cryptology - {CRYPTO} 2001},
volume={2139},
series={Lecture Notes in Computer Science},
editor={Kilian, Joe},
title={Identity-Based Encryption from the Weil Pairing},
publisher={Springer Berlin Heidelberg},
author={Boneh, Dan and Franklin, Matt},
pages={213-229},
}

@inproceedings{Clarke:2001:FN,
 author = {Clarke, Ian and Sandberg, Oskar and Wiley, Brandon and Hong, Theodore W.},
 title = {Freenet: A Distributed Anonymous Information Storage and Retrieval System},
 booktitle = {International Workshop on Designing Privacy Enhancing Technologies: Design Issues in Anonymity and Unobservability},
 year = {2001},
 pages = {46--66},
 numpages = {21},
 publisher = {Springer-Verlag New York, Inc.},
}

@incollection{Dingledine:2001:Reliability,
year={2001},
booktitle={Information Hiding},
volume={2137},
series={Lecture Notes in Computer Science},
editor={Moskowitz, IraS.},
title={A Reputation System to Increase {MIX-Net} Reliability},
publisher={Springer Berlin Heidelberg},
author={Dingledine, Roger and Freedman, MichaelJ. and Hopwood, David and Molnar, David},
pages={126-141},
}

@Inbook{Furukawa:2001:VerfiableShuffle,
author={Furukawa, Jun and Sako, Kazue},
editor={Kilian, Joe},
title={An Efficient Scheme for Proving a Shuffle},
bookTitle={Advances in Cryptology --- CRYPTO 2001: 21st Annual International Cryptology Conference, Santa Barbara, California, USA, August 19--23, 2001 Proceedings},
year={2001},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={368--387},
isbn={978-3-540-44647-7},
doi={10.1007/3-540-44647-8_22},
url={http://dx.doi.org/10.1007/3-540-44647-8_22}
}


@inproceedings{Jakobsson:2001:Robus-Mix,
 author = {Jakobsson, Markus and Juels, Ari},
 title = {An Optimally Robust Hybrid {Mix} Network},
 booktitle = {Proceedings of the Twentieth Annual {ACM} Symposium on Principles of Distributed Computing},
 series = {{PODC} '01},
 year = {2001},
 location = {Newport, Rhode Island, USA},
 pages = {284--292},
 numpages = {9},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@incollection{Jean:2001:Protocols:Survey,
year={2001},
booktitle={Designing Privacy Enhancing Technologies},
volume={2009},
series={Lecture Notes in Computer Science},
editor={Federrath, Hannes},
title={Traffic Analysis: Protocols, Attacks, Design Issues, and Open Problems},
publisher={Springer Berlin Heidelberg},
author={Jean{-}Fran{\c{c}}ois Raymond},
pages={10-29},
}

@inproceedings{Neff:2001:VSS,
 author = {Neff, C. Andrew},
 title = {A Verifiable Secret Shuffle and Its Application to e-Voting},
 booktitle = {Proceedings of the 8th ACM Conference on Computer and Communications Security},
 series = {CCS '01},
 year = {2001},
 isbn = {1-58113-385-5},
 location = {Philadelphia, PA, USA},
 pages = {116--125},
 numpages = {10},
 url = {http://doi.acm.org/10.1145/501983.502000},
 doi = {10.1145/501983.502000},
 acmid = {502000},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymous credentials, electronic voting, honest-verifier, mix-net, permutation, universal verifiability, verifiable mix, verifiable shuffle, zeroknowledge},
} 



@inproceedings{Rowstron:2001:Pastry,
 author = {Rowstron, Antony I. T. and Druschel, Peter},
 title = {Pastry: Scalable, Decentralized Object Location, and Routing for Large-Scale Peer-to-Peer Systems},
 booktitle = {Proceedings of the {IFIP/ACM} International Conference on Distributed Systems Platforms Heidelberg},
 series = {Middleware '01},
 year = {2001},
 pages = {329--350},
 numpages = {22},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
}

@Inbook{Shoup:1998:AnalysisTDH,
author={Shoup, Victor and Gennaro, Rosario},
editor={Nyberg, Kaisa},
title={Securing threshold cryptosystems against chosen ciphertext attack},
bookTitle={Advances in Cryptology --- EUROCRYPT'98: International Conference on the Theory and Application of Cryptographic Techniques Espoo, Finland, May 31 -- June 4, 1998 Proceedings},
year={1998},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={1--16},
isbn={978-3-540-69795-4},
doi={10.1007/BFb0054113},
url={http://dx.doi.org/10.1007/BFb0054113}
}


@inproceedings{Stoica:2001:Chord,
 author = {Stoica, Ion and Morris, Robert and Karger, David and Kaashoek, M. Frans and Balakrishnan, Hari},
 title = {Chord: A Scalable Peer-to-peer Lookup Service for Internet Applications},
 booktitle = {Proceedings of the 2001 Conference on Applications, Technologies, Architectures, and Protocols for Computer Communications},
 series = {{SIGCOMM} '01},
 year = {2001},
 pages = {149--160},
 numpages = {12},
 publisher = {ACM},
}

@incollection{Syverson:2001:OR-Security,
year={2001},
booktitle={Designing Privacy Enhancing Technologies},
volume={2009},
series={Lecture Notes in Computer Science},
editor={Federrath, Hannes},
title={Towards an Analysis of Onion Routing Security},
publisher={Springer Berlin Heidelberg},
author={Syverson, Paul and Tsudik, Gene and Reed, Michael and Landwehr, Carl},
pages={96-114},
}

@inproceedings{Waldman:2001:Tangler,
  author    = {Marc Waldman and
               David Mazi{\`{e}}res},
  title     = {Tangler: a censorship-resistant publishing system based on document
               entanglements},
  booktitle = {{CCS} 2001, Proceedings of the 8th {ACM} Conference on Computer and
               Communications Security, Philadelphia, Pennsylvania, USA, November
               6-8, 2001.},
  pages     = {126--135},
  year      = {2001}
}

@inproceedings{Berthold:2000,
  author    = {Oliver Berthold and
               Andreas Pfitzmann and
               Ronny Standtke},
  title     = {The Disadvantages of Free {MIX} Routes and how to Overcome Them},
  booktitle = {Designing Privacy Enhancing Technologies, International Workshop on
               Design Issues in Anonymity and Unobservability, Berkeley, CA, USA,
               July 25-26, 2000, Proceedings},
  year      = {2000},
  pages     = {30--45},

}

@inproceedings{Berthold:2000:JAP,
  author    = {Oliver Berthold and
               Hannes Federrath and
               Stefan K{\"{o}}psell},
  title     = {{Web MIXes}: A System for Anonymous and Unobservable Internet Access},
  booktitle = {Designing Privacy Enhancing Technologies, International Workshop on Design Issues in Anonymity and Unobservability, Berkeley, CA, USA, July 25-26, 2000, Proceedings},
  year      = {2000},
  pages     = {115--129},
}

@inproceedings{Berthold:2000:Anonymity,
 author = {Berthold, Oliver and Federrath, Hannes and K\"{o}hntopp, Marit},
 title = {Project Anonymity and Unobservability in the Internet},
 booktitle = {Proceedings of the Tenth Conference on Computers, Freedom and Privacy: Challenging the Assumptions},
 series = {{CFP} '00},
 year = {2000},
 location = {Toronto, Ontario, Canada},
 pages = {57--65},
 numpages = {9},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@incollection{Desmedt:2000:Break-Mix,
year={2000},
booktitle={Advances in Cryptology - {EUROCRYPT} 2000},
volume={1807},
series={Lecture Notes in Computer Science},
editor={Preneel, Bart},
title={How to Break a Practical {MIX} and Design a New One},
publisher={Springer Berlin Heidelberg},
author={Desmedt, Yvo and Kurosawa, Kaoru},
pages={557-572},
}

@inproceedings{Dingledine:2000:FreeHaven,
  author    = {Roger Dingledine and
               Michael J. Freedman and
               David Molnar},
  title     = {The Free Haven Project: Distributed Anonymous Storage Service},
  booktitle = {Designing Privacy Enhancing Technologies, International Workshop on
               Design Issues in Anonymity and Unobservability, Berkeley, CA, USA,
               July 25-26, 2000, Proceedings},
  pages     = {67--95},
  year      = {2000}
  }

@article{Dolev:2000:DCnet-XORTrees,
 author = {Dolev, Shlomi and Ostrobsky, Rafail},
 title = {Xor-trees for Efficient Anonymous Multicast and Reception},
 journal = {ACM Trans. Inf. Syst. Secur.},
 issue_date = {May 2000},
 volume = {3},
 number = {2},
 month = {may},
 year = {2000},
 issn = {1094-9224},
 pages = {63--84},
 numpages = {22},
 url = {http://doi.acm.org/10.1145/354876.354877},
 doi = {10.1145/354876.354877},
 acmid = {354877},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {anonymous communication, anonymous multicast},
} 

@inproceedings{Kleinberg:2000:SWM,
 author = {Kleinberg, Jon},
 title = {The Small-world Phenomenon: An Algorithmic Perspective},
 booktitle = {Proceedings of the Thirty-second Annual {ACM} Symposium on Theory of Computing},
 series = {{STOC} '00},
 year = {2000},
 pages = {163--170},
 numpages = {8},
 publisher = {ACM},
}

@incollection{Mitomo:2000:Mix-Attack,
year={2000},
booktitle={Advances in Cryptology - {ASIACRYPT} 2000},
volume={1976},
series={Lecture Notes in Computer Science},
editor={Okamoto, Tatsuaki},
title={Attack for Flash {MIX}},
publisher={Springer Berlin Heidelberg},
author={Mitomo, Masashi and Kurosawa, Kaoru},
pages={192-204},
}

@inproceedings{Pfitzmann:2000:terminology,
  author    = {Andreas Pfitzmann and
               Marit K{\"{o}}hntopp},
  title     = {Anonymity, Unobservability, and Pseudonymity - {A} Proposal for Terminology},
  booktitle = {Designing Privacy Enhancing Technologies, International Workshop on Design Issues in Anonymity and Unobservability, Berkeley, CA, USA, July 25-26, 2000, Proceedings},
  year      = {2000},
  pages     = {1--9}
}

@inproceedings{Raymond:2000:Survey,
  author    = {Jean{-}Fran{\c{c}}ois Raymond},
  title     = {Traffic Analysis: Protocols, Attacks, Design Issues, and Open Problems},
  booktitle = {Designing Privacy Enhancing Technologies, International Workshop on
               Design Issues in Anonymity and Unobservability, Berkeley, CA, USA,
               July 25-26, 2000, Proceedings},
  year      = {2000},
  pages     = {10--29},
}

@inproceedings{Shields:2000:hordes,
 author = {Shields, Clay and Levine, Brian Neil},
 title = {A Protocol for Anonymous Communication over the Internet},
 booktitle = {Proceedings of the 7th {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '00},
 year = {2000},
 location = {Athens, Greece},
 pages = {33--42},
 numpages = {10},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@inproceedings{Thorup:2000:SUH,
  author    = {Mikkel Thorup},
  title     = {Even strongly universal hashing is pretty fast},
  booktitle = {Proceedings of the Eleventh Annual {ACM-SIAM} Symposium on Discrete
               Algorithms, January 9-11, 2000, San Francisco, CA, {USA.}},
  pages     = {496--497},
  year      = {2000},
  crossref  = {DBLP:conf/soda/2000},
  url       = {http://dl.acm.org/citation.cfm?id=338219.338597},
  timestamp = {Fri, 07 Dec 2012 17:02:09 +0100},
  biburl    = {http://dblp.uni-trier.de/rec/bib/conf/soda/Thorup00},
  bibsource = {dblp computer science bibliography, http://dblp.org}
}


@inproceedings{Waldman:2000:Publius,
  author    = {Marc Waldman and
               Aviel D. Rubin and
               Lorrie Faith Cranor},
  title     = {Publius: {A} Robust, Tamper-Evident, Censorship-Resistant, and Source-Anonymous
               Web Publishing System},
  booktitle = {9th {USENIX} Security Symposium, Denver, Colorado, USA, August 14-17,
               2000},
}

@inproceedings{NameDropper:1999,
	author    = {Mor Harchol{-}Balter and
	Frank Thomson Leighton and
	Daniel Lewin},
	title     = {Resource Discovery in Distributed Networks},
	booktitle = {Proceedings of the Eighteenth Annual {ACM} Symposium on Principles of Distributed Computing},
	series = {PODC '99},
	pages     = {229--237},
	year      = {1999}
}

@inproceedings{Castro:1999:BFT,
  title={Practical Byzantine fault tolerance},
  author={Castro, Miguel and Liskov, Barbara and others},
  booktitle={{OSDI}},
  volume={99},
  pages={173--186},
  year={1999}
}

@misc{Feeney:1999:routingtaxonomy,
author = {Laura Marie Feeney},
title = {{A Taxonomy for Routing Protocols in Mobile Ad Hoc Networks}},
year = {1999},
}



@misc{Shostack:1999:Freedom,
  title={Freedom 1.0 security issues and analysis},
  author={Shostack, Adam and Goldberg, Ian},
  year={1999},
  publisher={November}
}

@Inbook{Gennaro:1999:DistKeyGen,
author={Gennaro, Rosario
and Jarecki, Stanis{\l}aw
and Krawczyk, Hugo
and Rabin, Tal},
editor={Stern, Jacques},
title={Secure Distributed Key Generation for Discrete-Log Based Cryptosystems},
bookTitle={Advances in Cryptology --- EUROCRYPT '99: International Conference on the Theory and Application of Cryptographic Techniques Prague, Czech Republic, May 2--6, 1999 Proceedings},
year={1999},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={295--310},
isbn={978-3-540-48910-8},
doi={10.1007/3-540-48910-X_21},
url={http://dx.doi.org/10.1007/3-540-48910-X_21}
}

@inproceedings{Jakobsson:1999:Flash-Mix,
 author = {Jakobsson, Markus},
 title = {Flash Mixing},
 booktitle = {Proceedings of the Eighteenth Annual {ACM} Symposium on Principles of Distributed Computing},
 series = {{PODC} '99},
 year = {1999},
 location = {Atlanta, Georgia, USA},
 pages = {83--89},
 numpages = {7},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@incollection{Abe:1998:Mixnets,
year={1998},
booktitle={Advances in Cryptology - {EUROCRYPT} '98},
volume={1403},
series={Lecture Notes in Computer Science},
editor={Nyberg, Kaisa},
title={Universally verifiable mix-net with verification work independent of the number of mix-servers},
publisher={Springer Berlin Heidelberg},
author={Abe, Masayuki},
pages={437-447},
}

@incollection{Jakobsson:1998:Mix,
year={1998},
booktitle={Advances in Cryptology - {EUROCRYPT} '98},
volume={1403},
series={Lecture Notes in Computer Science},
editor={Nyberg, Kaisa},
title={A practical mix},
publisher={Springer Berlin Heidelberg},
author={Jakobsson, Markus},
pages={448-461},
}


@inproceedings{Kesdogan:1998:stopandgo,
  author    = {Dogan Kesdogan and
               Jan Egner and
               Roland B{\"{u}}schkes},
  title     = {{Stop-and-Go-MIXes} Providing Probabilistic Anonymity in an Open System},
  booktitle = {Information Hiding, Second International Workshop, Portland, Oregon, USA, April 14-17, 1998, Proceedings},
  year      = {1998},
  pages     = {83--98}
}

@ARTICLE{Reed:1998:Onion-Routing, 
author={Reed, M.G. and Syverson, P.F. and Goldschlag, D.M.}, 
journal={Selected Areas in Communications, {IEEE} Journal on}, 
title={Anonymous connections and onion routing}, 
year={1998}, 
month={May}, 
volume={16}, 
number={4}, 
pages={482-494},
}

@article{Reiter:1998:Crowds,
 author = {Reiter, Michael K. and Rubin, Aviel D.},
 title = {Crowds: Anonymity for Web Transactions},
 journal = {ACM Trans. Inf. Syst. Secur.},
 volume = {1},
 number = {1},
 month = {November},
 year = {1998},
 pages = {66--92},
 numpages = {27},
 publisher = {ACM},
}

@article{Jerichow:1998:realtimemix,
  author    = {Anja Jerichow and
               Jan M{\"{u}}ller and
               Andreas Pfitzmann and
               Birgit Pfitzmann and
               Michael Waidner},
  title     = {Real-time mixes: a bandwidth-efficient anonymity protocol},
  journal   = {{IEEE} Journal on Selected Areas in Communications},
  volume    = {16},
  number    = {4},
  pages     = {495--509},
  year      = {1998}
}

@inproceedings{Cramer:1997:DistributedCrypto,
 author = {Cramer, Ronald and Gennaro, Rosario and Schoenmakers, Berry},
 title = {A Secure and Optimally Efficient Multi-authority Election Scheme},
 booktitle = {Proceedings of the 16th Annual International Conference on Theory and Application of Cryptographic Techniques},
 series = {EUROCRYPT'97},
 year = {1997},
 isbn = {3-540-62975-0},
 location = {Konstanz, Germany},
 pages = {103--118},
 numpages = {16},
 url = {http://dl.acm.org/citation.cfm?id=1754542.1754554},
 acmid = {1754554},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 

@misc{Helmers:1997:anon, 
	author = {Sabine Helmers},
	title = {A Brief History of anon.penet.fi - The Legendary Anonymous Remailer},
	month = {September},
	year = {1997},
	howpublished = {\url{http://www.december.com/cmc/mag/1997/sep/helmers.html}},
	note = {Last accessed: August 05, 2015}
}

@inproceedings{Cramer:1997:SOE,
 author = {Cramer, Ronald and Gennaro, Rosario and Schoenmakers, Berry},
 title = {A Secure and Optimally Efficient Multi-authority Election Scheme},
 booktitle = {Proceedings of the 16th Annual International Conference on Theory and Application of Cryptographic Techniques},
 series = {EUROCRYPT'97},
 year = {1997},
 isbn = {3-540-62975-0},
 location = {Konstanz, Germany},
 pages = {103--118},
 numpages = {16},
 url = {http://dl.acm.org/citation.cfm?id=1754542.1754554},
 acmid = {1754554},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 



@article{Syverson:1997:PWB,
 author = {Syverson, Paul F. and Reed, Michael G. and Goldschlag, David M.},
 title = {Private Web Browsing},
 journal = {J. Comput. Secur.},
 issue_date = {June 1997},
 volume = {5},
 number = {3},
 month = jun,
 year = {1997},
 issn = {0926-227X},
 pages = {237--248},
 numpages = {12},
 url = {http://dl.acm.org/citation.cfm?id=353686.353689},
 acmid = {353689},
 publisher = {IOS Press},
 address = {Amsterdam, The Netherlands, The Netherlands},
 keywords = {anonymity, privacy, security, traffic analysis},
} 



@inproceedings{Goldschlag:1996:onionrouting,
year={1996},
booktitle={Information Hiding},
volume={1174},
series={Lecture Notes in Computer Science},
editor={Anderson, Ross},
title={Hiding Routing information},
publisher={Springer Berlin Heidelberg},
author={Goldschlag, DavidM. and Reed, MichaelG. and Syverson, PaulF.},
pages={137-150},
}

@inproceedings{Babel:1996,
  author    = {Ceki G{\"{u}}lc{\"{u}} and
               Gene Tsudik},
  title     = {Mixing Email with Babel},
  booktitle = {1996 Symposium on Network and Distributed System Security, {NDSS} '96, San Diego, CA, February 22-23, 1996},
  year      = {1996},
  pages     = {2--16},
}

@article{Dai:1996:PipeNet,
  title={PipeNet 1.1},
  author={Dai, Wei},
  journal={Usenet post},
  month = {August},
  year={1996}
}

@article{Parekh:1996,
  author    = {Sameer Parekh},
  title     = {Prospects for Remailers},
  journal   = {First Monday},
  year      = {1996},
  volume    = {1},
  number    = {2},
  url       = {http://firstmonday.org/htbin/cgiwrap/bin/ojs/index.php/fm/article/view/476},
}

@inproceedings{Reed:1996:Proxies,
  author    = {Michael G. Reed and
               Paul F. Syverson and
               David M. Goldschlag},
  title     = {Proxies For Anonymous Routing},
  booktitle = {13th Annual Computer Security Applications Conference {(ACSAC)} 1996),
               9-13 December 1996, San Diego, CA, {USA}},
  pages     = {95--104},
  year      = {1996},
  crossref  = {DBLP:conf/acsac/1996},
}

@inproceedings{Guklu:1996:Babel,
  author    = {Ceki G{\"{u}}lc{\"{u}} and
               Gene Tsudik},
  title     = {Mixing Email with Babel},
  booktitle = {1996 Symposium on Network and Distributed System Security, {NDSS} '96, San Diego, CA, February 22-23, 1996},
  year      = {1996},
  pages     = {2--16},
}

@proceedings{DBLP:conf/acsac/1996,
  title     = {13th Annual Computer Security Applications Conference {(ACSAC} 1996),
               9-13 December 1996, San Diego, CA, {USA}},
  publisher = {{IEEE} Computer Society},
  year      = {1996},
}

@inproceedings{Sako:1995:Voting,
  author    = {Kazue Sako and
               Joe Kilian},
  title     = {Receipt-Free {Mix-Type} Voting Scheme - {A} Practical Solution to the
               Implementation of a Voting Booth},
  booktitle = {Advances in Cryptology - {EUROCRYPT} '95, International Conference
               on the Theory and Application of Cryptographic Techniques, Saint-Malo,
               France, May 21-25, 1995, Proceeding},
  pages     = {393--403},
  year      = {1995}
}

@inproceedings{Kung:1994:N23,
 author = {Kung, H. T. and Blackwell, Trevor and Chapman, Alan},
 title = {Credit-based Flow Control for ATM Networks: Credit Update Protocol, Adaptive Credit Allocation and Statistical Multiplexing},
 booktitle = {Proceedings of the Conference on Communications Architectures, Protocols and Applications},
 series = {{SIGCOMM} '94},
 year = {1994},
 location = {London, United Kingdom},
 pages = {101--114},
 numpages = {14},
 publisher = {ACM},
 address = {New York, NY, USA},
}

@Inbook{Fujioka:1993:voting,
author={Fujioka, Atsushi
and Okamoto, Tatsuaki
and Ohta, Kazuo},
editor={Seberry, Jennifer
and Zheng, Yuliang},
title={A practical secret voting scheme for large scale elections},
bookTitle={Advances in Cryptology --- AUSCRYPT '92: Workshop on the Theory and Application of Cryptographic Techniques Gold Coast, Queensland, Australia, December 13--16, 1992 Proceedings},
year={1993},
publisher={Springer Berlin Heidelberg},
address={Berlin, Heidelberg},
pages={244--251},
isbn={978-3-540-47976-5},
doi={10.1007/3-540-57220-1_66},
url={http://dx.doi.org/10.1007/3-540-57220-1_66}
}


@inproceedings{Bellare:1993:RO,
 author = {Bellare, Mihir and Rogaway, Phillip},
 title = {Random Oracles Are Practical: A Paradigm for Designing Efficient Protocols},
 booktitle = {Proceedings of the 1st {ACM} Conference on Computer and Communications Security},
 series = {{CCS} '93},
 year = {1993},
 pages = {62--73},
 numpages = {12},
 publisher = {ACM},
}

@inproceedings{Pedersen:1991:DKG,
 author = {Pedersen, Torben P.},
 title = {Non-Interactive and Information-Theoretic Secure Verifiable Secret Sharing},
 booktitle = {Proceedings of the 11th Annual International Cryptology Conference on Advances in Cryptology},
 series = {CRYPTO '91},
 year = {1992},
 isbn = {3-540-55188-3},
 pages = {129--140},
 numpages = {12},
 url = {http://dl.acm.org/citation.cfm?id=646756.705507},
 acmid = {705507},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
} 


@inproceedings{Pedersen:1991:TCWithoutDealer,
 author = {Pedersen, Torben Pryds},
 title = {A Threshold Cryptosystem Without a Trusted Party},
 booktitle = {Proceedings of the 10th Annual International Conference on Theory and Application of Cryptographic Techniques},
 series = {EUROCRYPT'91},
 year = {1991},
 isbn = {3-540-54620-0},
 location = {Brighton, UK},
 pages = {522--526},
 numpages = {5},
 url = {http://dl.acm.org/citation.cfm?id=1754868.1754929},
 acmid = {1754929},
 publisher = {Springer-Verlag},
 address = {Berlin, Heidelberg},
} 




@incollection{Pfitzmann:1991:ISDN-MIXes,
year={1991},
booktitle={Kommunikation in verteilten Systemen},
volume={267},
series={Informatik-Fachberichte},
title={ISDN-Mixes: Untraceable Communication with Very Small Bandwidth Overhead},
publisher={Springer Berlin Heidelberg},
author={Pfitzmann, Andreas and Pfitzmann, Birgit and Waidner, Michael},
pages={451-463},
}

@incollection{Bos:1990:DC-Disrupters,
year={1990},
booktitle={Advances in Cryptology - {EUROCRYPT} '89},
volume={434},
series={Lecture Notes in Computer Science},
editor={Quisquater, Jean-Jacques and Vandewalle, Joos},
title={Detection of Disrupters in the DC Protocol},
publisher={Springer Berlin Heidelberg},
author={Bos, Jurjen and den Boer, Bert},
pages={320-327},
}

@inproceedings{Pfitzmann:1990:Pfitzmann,
  author    = {Birgit Pfitzmann and
               Andreas Pfitzmann},
  title     = {How to Break the Direct {RSA}-Implementation of {Mixes}},
  booktitle = {Advances in Cryptology - {EUROCRYPT} '89, Workshop on the Theory and Application of of Cryptographic Techniques, Houthalen, Belgium, April 10-13, 1989, Proceedings},
  year      = {1989},
  pages     = {373--381}
}

@incollection{Waidner:1990:DC,
year={1990},
booktitle={Advances in Cryptology - {EUROCRYPT} '89},
volume={434},
series={Lecture Notes in Computer Science},
editor={Quisquater, Jean-Jacques and Vandewalle, Joos},
title={The Dining Cryptographers in the Disco: Unconditional Sender and Recipient Untraceability with Computationally Secure Serviceability},
publisher={Springer Berlin Heidelberg},
author={Waidner, Michael and Pfitzmann, Birgit},
pages={690-690},
}

@incollection{Waidner:1990:Attack,
year={1990},
booktitle={Advances in Cryptology - {EUROCRYPT} '89},
volume={434},
series={Lecture Notes in Computer Science},
editor={Quisquater, Jean-Jacques and Vandewalle, Joos},
title={Unconditional Sender and Recipient Untraceability in Spite of Active Attacks},
publisher={Springer Berlin Heidelberg},
author={Waidner, Michael},
pages={302-319},
}

@inproceedings{Desmedt:1989:TC,
 author = {Desmedt, Yvo G. and Frankel, Yair},
 title = {Threshold Cryptosystems},
 booktitle = {Proceedings on Advances in Cryptology},
 series = {CRYPTO '89},
 year = {1989},
 isbn = {0-387-97317-6},
 location = {Santa Barbara, California, USA},
 pages = {307--315},
 numpages = {9},
 url = {http://dl.acm.org/citation.cfm?id=118209.118237},
 acmid = {118237},
 publisher = {Springer-Verlag New York, Inc.},
 address = {New York, NY, USA},
 keywords = {authentication, cryptography, digital signatures, electronic funds transfer, electronic signatures, public key cryptosystem, receipts},
} 

@inproceedings{Schnorr:1989:Signatures,
 author = {Schnorr, Claus-Peter},
 title = {Efficient Identification and Signatures for Smart Cards},
 booktitle = {Proceedings of the 9th Annual International Cryptology Conference on Advances in Cryptology},
 series = {CRYPTO '89},
 year = {1990},
 isbn = {3-540-97317-6},
 pages = {239--252},
 numpages = {14},
 url = {http://dl.acm.org/citation.cfm?id=646754.705037},
 acmid = {705037},
 publisher = {Springer-Verlag},
 address = {London, UK, UK},
} 

@article{Chaum:1988:DCNets,
year={1988},
journal={Journal of Cryptology},
volume={1},
number={1},
title={The dining cryptographers problem: Unconditional sender and recipient untraceability},
publisher={Springer-Verlag},
author={Chaum, David},
pages={65-75},
}

@ARTICLE{Bell:1986:routingreview, 
author={Bell, P. and Jabbour, K.}, 
journal={Communications Magazine, IEEE}, 
title={Review of point-to-point network routing algorithms}, 
year={1986}, 
month={January}, 
volume={24}, 
number={1}, 
pages={34-38}, 
}

@inproceedings{Cleve:1986:BiasCoinToss,
 author = {Cleve, Richard},
 title = {Limits on the Security of Coin Flips when Half the Processors Are Faulty},
 booktitle = {Proceedings of the Eighteenth Annual ACM Symposium on Theory of Computing},
 series = {STOC '86},
 year = {1986},
 isbn = {0-89791-193-8},
 location = {Berkeley, California, USA},
 pages = {364--369},
 numpages = {6},
 url = {http://doi.acm.org/10.1145/12130.12168},
 doi = {10.1145/12130.12168},
 acmid = {12168},
 publisher = {ACM},
 address = {New York, NY, USA},
} 



@incollection{Pfitzmann:1986:Unobservability,
year={1986},
booktitle={Advances in Cryptology - {EUROCRYPT} '85},
volume={219},
series={Lecture Notes in Computer Science},
editor={Pichler, Franz},
title={Networks Without User Observability - Design Options},
publisher={Springer Berlin Heidelberg},
author={Pfitzmann, Andreas and Waidner, Michael},
pages={245-253},
}

@incollection{ElGamal:1985,
year={1985},
booktitle={Advances in Cryptology},
volume={196},
series={Lecture Notes in Computer Science},
editor={Blakley, GeorgeRobert and Chaum, David},
title={A Public Key Cryptosystem and a Signature Scheme Based on Discrete Logarithms},
publisher={Springer Berlin Heidelberg},
author={ElGamal, Taher},
pages={10-18},
}

@article{Blum:1983:CoinFlipping,
 author = {Blum, Manuel},
 title = {Coin Flipping by Telephone a Protocol for Solving Impossible Problems},
 journal = {SIGACT News},
 issue_date = {Winter-Spring 1983},
 volume = {15},
 number = {1},
 month = jan,
 year = {1983},
 issn = {0163-5700},
 pages = {23--27},
 numpages = {5},
 url = {http://doi.acm.org/10.1145/1008908.1008911},
 doi = {10.1145/1008908.1008911},
 acmid = {1008911},
 publisher = {ACM},
 address = {New York, NY, USA},
} 

@article{Chaum:1981:mixnets,
  author    = {David Chaum},
  title     = {Untraceable Electronic Mail, Return Addresses, and Digital Pseudonyms},
  journal   = {Commun. {ACM}},
  year      = {1981},
  volume    = {24},
  number    = {2},
  pages     = {84--88},
}

@article{Postel:1981:TCP,
  title={Transmission control protocol},
  author={Postel, Jon},
  year={1981}
}


@article{Shamir:1979:SS,
 author = {Shamir, Adi},
 title = {How to Share a Secret},
 journal = {Commun. ACM},
 issue_date = {Nov. 1979},
 volume = {22},
 number = {11},
 month = nov,
 year = {1979},
 issn = {0001-0782},
 pages = {612--613},
 numpages = {2},
 url = {http://doi.acm.org/10.1145/359168.359176},
 doi = {10.1145/359168.359176},
 acmid = {359176},
 publisher = {ACM},
 address = {New York, NY, USA},
 keywords = {cryptography, interpolation, key management},
} 


@article{Merkle:1978:SC,
 author = {Merkle, Ralph C.},
 title = {Secure Communications over Insecure Channels},
 journal = {Commun. ACM},
 year={1978}, 
 month={April}, 
 volume = {21},
 number = {4},
 pages = {294--299},
 numpages = {6},
}

@ARTICLE{Diffie:1976:DH, 
author={Diffie, W. and Hellman, M.E.}, 
journal={Information Theory, IEEE Transactions on}, 
title={New directions in cryptography},
year={1976}, 
month={November}, 
volume={22}, 
number={6}, 
pages={644-654}
}

@article{Bloom:1970:BloomFilter,
 author = {Bloom, Burton H.},
 title = {Space/Time Trade-offs in Hash Coding with Allowable Errors},
 journal = {Commun. ACM},
 issue_date = {July 1970},
 volume = {13},
 number = {7},
 month = {jul},
 year = {1970},
 issn = {0001-0782},
 pages = {422--426},
 numpages = {5},
 publisher = {ACM},
 address = {New York, NY, USA},
}

